Scheduling under Non-Uniform Job and Machine Delays

We study the problem of scheduling precedence-constrained jobs on heterogenous machines in the presence of non-uniform job and machine communication delays. We are given as input $n$ unit size precedence-ordered jobs and $m$ related machines such that machine $i$ can execute up to $m_i$ jobs at a time. Each machine $i$ has an in-delay $\rho^{\mathrm{in}}_i$ and out-delay $\rho^{\mathrm{out}}_i$. Likewise, each job $v$ has an in-delay $\rho^{\mathrm{in}}_v$ and out-delay $\rho^{\mathrm{out}}_v$. In a schedule, job $v$ may be executed on machine $i$ at time $t$ if each predecessor $u$ of $v$ is completed on $i$ before time $t$ or on any machine $j$ before time $t - (\rho^{\mathrm{in}}_i + \rho^{\mathrm{out}}_j + \rho^{\mathrm{out}}_u + \rho^{\mathrm{in}}_v)$. The goal is to construct a schedule that minimizes makespan. We consider schedules that allow duplication of jobs as well as schedules which do not. When duplication is allowed, we provide an asymptotic $\mathrm{polylog}(n)$-approximation algorithms both when duplication is allowed and when it is not. We also obtain a true $\mathrm{polylog}(n)$-approximation for symmetric machine and job delays. These are the first polylogarithmic approximation algorithms for scheduling with non-uniform communication delays. We also consider a more general model, where the delay can be an arbitrary function of the job and the machine executing it: job $v$ can be executed on machine $i$ at time $t$ if all of $v$'s predecessors are executed on $i$ by time $t-1$ or on any machine by time $t - \rho_{v,i}$. We present an approximation-preserving reduction from the Unique Machines Precedence-constrained Scheduling (UMPS) problem, first defined in [DKRSTZ22], to this job-machine delay model. The reduction entails logarithmic hardness for this delay setting, as well as polynomial hardness if the conjectured hardness of UMPS holds.

==> SODA 23/SODA23_rebuttal <==
We thank the reviewers for their insightful comments. Our responses below are organized by topic area. 

**High-level Comments on Technical Contributions**

In addition to the algorithmic results mentioned by the reviewers, we believe that one of our primary contributions is to open up the non-uniform delay problem space. Prior to our paper, the only results for non-uniform delay were hardness results due to Davies et al (citation [12] in submission). The fact that polylogarithmic approximations are possible for fairly general models in this space seems to us an important discovery. Also, we find it compelling that this was done with a standard linear programming framework, though the LP itself is carefully crafted for our problem. We believe that the simplicity of this framework is important in inviting future research.

**Technical Comparison with Prior Work (Review 1)**

In our revision, we will provide a more detailed comparison with previous work, specifically with the rounding procedure used in Maiti et al (MRSSV, citation [28] in submission). The MRSSV procedure selects an ordering of machines such that the capacity of machine groups decreases as the speed increases. Each job is then placed on the group of machines for which the LP executes at least half the job's mass on slower (higher capacity) groups. For MRSSV, this rounding avoids the need to track the load of duplicated jobs because the ordering of groups itself encodes information about the relative speeds and capacities of the groups. 

The introduction of in- and out-delays presents significant challenges in finding a suitable ordering on machine groups. To address this issue, we perform a simpler rounding where jobs are placed on the machine group for which the LP maximizes the job's mass. However, implementing this simplified rounding poses its own problems since we have no information about the relative capabilities of machine groups, causing the amount of duplication necessary to approximate the LP makespan to be extremely high compared to the MRSSV LP load. Therefore, we enhance our LP to directly track the amount of duplication done on each machine group.  A key attraction of this new approach is that we are able to generalize the result to variable speeds and processors through additional constraints. This significantly generalizes the results of MRSSV using a simpler rounding procedure with a more sophisticated LP.

We re-emphasize that the technical apparatus is only one aspect of our main contribution, the other being to provide the first positive results for non-uniform communication delay. We believe our framework paves the way for future work in this space, possibly toward progress in other non-uniform delay models. 

**Metric Delays (Review 2)**

We address the question about what is known for metric delays.  Our results are the first known upper bounds for any model with non-uniform (metric or otherwise) machine delays.  As mentioned above, the only known result in approximability for non-uniform delays is due to Davies et al, who present a logarithmic-hardness result for job dependent delays and conjecture a greater hardness factor for the same.  Our positive results counterbalance these hardness results and help carve out the space of scheduling with non-uniform delays.   

We note that our methods do not immediately imply a result for general metric machine delays.  As illustrated in Figure 2, however, our machine dependent model includes scenarios where the delays are not even metric. We find it surprising that polylogarithmic approximations exist for such asymmetric cases. 

**Improvement to Technical Writing (Review 3)**

The suggestion to present a simplified result first is well taken. We considered writing an initial section where we discussed the uniform speed, size setting, but decided against it so that we could present the full algorithm in the first ten pages of the paper. We agree that presenting uniform speed and size first would aid in comphrension, and the final version can be restructured to present this result first, before generalizing to the full model. 

**Minor Comments**

All minor comments will be corrected in our final revision. Reviewer 1 is correct that Lemma 2.1 holds only in the case where we require initial and final communication phases for each machine, and this will be corrected as well. Removing this assumption incurs an additive loss of $\Delta_\sigma$, which does not affect our final result.

==> SODA 23/dedup.tex <==
\section{Approximation algorithms for no-duplication schedules}

In this section, we consider no-duplication schedules and prove \Cref{thm:mdps-no-dup} in \Cref{sec:mdps-no-dup} and \Cref{thm:mdps-symmetric-no-dup} in \Cref{sec:mdps-symmetric-no-dup}.

\subsection{Machine-dependent delays}
\label{sec:mdps-no-dup}
Our algorithm for no-duplication schedules first runs Algorithm~\ref{alg:scheduler_jm} for the problem, which produces a schedule (with possible duplications) having a structure illustrated in Figure~\ref{fig:schedule_structure}.  By line 7 of Algorithm~\ref{alg:scheduler_jm}, the schedule $\sigma_{k,d}$ for each $V_{k,d}$ includes a delay of $\bar{\rho}_k$ at the start.  We next 
convert the schedule $\sigma_{k,d}$, for each $V_{k,d}$, to a no-duplication schedule using the following lemma from \cite{maiti_etal.commdelaydup_FOCS.20}.  
\begin{lemma}[Restatement of Theorem 3 from \cite{maiti_etal.commdelaydup_FOCS.20}]
  Given a \udps\ instance where the delay is \(\rho\) and a schedule of length \(D \geq \rho\), there is a polynomial time algorithm that  computes a no-duplication schedule for the instance with length \(O((\log m )(\log n)^{2}D)\).
  \label{lemma:focs}
\end{lemma}
If the no-duplication schedule thus computed for \(V_{k,d}\) does not have a initial delay \(\bar{\rho}_k\), then we introduce a delay of $\bar{\rho}_k$ at the start of the schedule.  Let $\hat{\sigma}_{v,k}$ denote the no-duplication schedule thus computed for \(V_{k,d}\).  We concatenate the $\hat{\sigma}_{v,k}$ in the order specified in Figure~\ref{fig:schedule_structure}.  By construction, there is no duplication of jobs within any $\hat{\sigma}_{v,k}$.  To ensure that the final schedule has no duplication, we keep the first occurrence of each job in the schedule, and prune all duplicate occurrences.  We now show that no precedence constraints are violated.
\begin{lemma}
  In the above algorithm, all precedence constraints are satisfied.
  \label{lem:de-dup-constraints}
\end{lemma}

\begin{proof}
  Suppose \(u \prec v\). Pruning of a duplicate copy of $u$ can only cause a precedence violation if the copy of \(u\) that \(v\) waits for is pruned, so we assume \(u\) is pruned. For each copy of \(v\) scheduled on some machine \(i\), either some copy of \(u\) is also scheduled on \(i\), or it needs to wait \(\rho_{i}\) time to wait for those completed on other machines to be transmitted. In the former case, \(u\) will only be pruned if it is not the first occurrence. This can only happen if the first occurrence of \(u\) is in an earlier \(V_{k, d}\), since our subroutine guarantees that there is no duplication within a \(V_{k, d}\). Due to our in-delay model, as long as a later occurrence of \(u\) can be transmitted in time, so can all its previous occurrences. Therefore a copy of \(u\) will be available to \(v\). In the latter case, either \(u\) is within the same \(V_{k, d}\), or is in a previous one. In either case, the earlier occurrences of \(u\) have to be in earlier \(V_{k, d}\), and will be available to \(v\).  So the pruning of this copy of $u$ will not cause a precedence violation.
\end{proof}

\begin{theorem}
There exists a polynomial time algorithm that produces a no-duplication schedule whose makespan is at most $\polylog(n) (\makespan{\sigma} + \delay{\sigma}))$ for any schedule $\sigma$.
\end{theorem}

\begin{proof}
  Lemma~\ref{lem:de-dup-constraints} establishes the feasibility of the schedule. By definition, each job is scheduled exactly once. It remains to bound the approximation ratio.  Let \(\tau_{k, d}\) be the makespan of the schedule of \(V_{k, d}\) given by the subroutine we use on line 6 of \Cref{alg:scheduler}, and \(\tau_{k, d}'\) be the makespan of the de-duplicated version. Then \Cref{lemma:focs} shows that \(\tau_{k, d}' \leq O((\log n_{k, d})^{2}(\log m)(\tau_{k, d} + \rho_{k}))\), where \(n_{k, d}\) is the number of jobs in \(V_{k, d}\), which is upper bounded by \(n\).  There are at most \(n\) jobs to schedule, so having more than \(n\) machines does not help us, therefore we can assume \(m \leq n\) without loss of generality. \Cref{alg:uniform} guarantees that there is at least an in-delay at the start of \(\tau_{k, d}\), so \(\tau_{k, d} \geq \rho_{k}\), therefore \(\tau_{k, d}' \leq O((\log n_{k, d})^{3}\tau_{k, d})\).
   Therefore, the total makespan
  \[\sum_{k, d}\tau_{k, d}' \leq \sum_{k, d}O((\log n)^{3}\tau_{k, d})  \leq O((\log n)^{3}) \cdot \sum_{k, d}\tau_{k, d} = O(\text{polylog}(n) \makespan{\sigma} + \delay{\sigma}))\]
\end{proof}

\subsection{Symmetric delays}
\label{sec:mdps-symmetric-no-dup}
In this section, we establish a true polylogarithmic approximation for the no-duplication model if the delays are symmetric, i.e., \(\delayin i = \delayout i\).  The additive term of delay in Theorems~\ref{thm:mdps} and~\ref{thm:mdps-no-dup} comes from \Cref{alg:uniform}, where to ensure all previously scheduled jobs are available, we insert a suitable delay at the front.  This can be a cost too high if, for instance, the optimal solution does not incur any communication 
into a particular group and yet uses machines in the group to process jobs.  To overcome this difficulty, we develop a method that, given an upper bound $T$ on the optimal makespan, determines which groups participate in an approximately optimal solution without any communication.  Formally, we establish the following lemma which, together with a binary search on $T$, yields  \Cref{thm:mdps-symmetric-no-dup}.
\begin{lemma}
\label{lem:mdps-symmetric-no-dup}
There exists a polynomial time algorithm such that given \(T\), either gives a schedule of length \(O(\polylog (n)T)\), or asserts that \(\opt > T\).
\end{lemma}

Let \(S\) (resp., $S'$) be the set of machines that have delay at most (resp., larger than) \(T\).  
Let $G$ denote the DAG defined by the set of jobs and its precedence constraints.  Let $G'$ denote the undirected graph obtained from $G$ by removing directions from all edges.  Under symmetric delays,  we can afford no communication in either direction with machines in \(S'\), so in the absence of duplication both \opt\  and our algorithm will only schedule full connected components of $G'$ on \(S'\).  A priori, it is unclear how to distribute the connected components among $S$ and $S'$.  We revise the LP framework of Section~\ref{sec:approx-mdps} so that it guides this distribution while yielding a fractional placement without duplication on $S'$ and a fractional placement with duplication on $S$.  We then show how to design a full no-duplication schedule from these fractional placements.

For each connected component \(d\) and each machine \(i\in S'\), we define an LP variable \(X_{d, i}\), indicating whether the component is scheduled on machine \(i\). Therefore for the completion of jobs, we replace constraint~\labelcref{LP:execution} with
\begin{equation}
  \label{LP:execution_dedup_simple}
\sum_{k} x_{v, k} + \sum_{i\in S'} X_{d, i} = 1, \quad \forall d, \forall v\in d
\end{equation}
Use \(w(d)\) to denote the total number of jobs in connected component \(d\), and \(L(d)\) the length of its critical path. We also need to add the following constraints:
\begin{align}
  &D\geq \sum_{d}\frac{X_{d, i}\cdot w(d)}{m_{i}s_{i}}, &&\forall i \label{LP:makespan_Xdi}\\
  &0 \leq X_{d, i} \leq 1, &&\forall d, i \label{LP:Xdi}\\
  &X_{d, i} = 0, &&\forall d, \text{ if } l(d) > s_{i}\cdot T \label{LP:Xdi:critical}\\
  &X_{d, i} = 0, &&\forall d, \text{ if } w(d) > m_{i}\cdot s_{i}\cdot T \label{LP:Xdi:load}
\end{align}

After solving the LP, if \(D > T\), we know \textsf{OPT} cannot have a schedule less than \(T\), since a no-duplication schedule is also a valid with-duplication schedule, and satisfies the revised LP. If \(D \leq T\), we proceed to round and give a schedule. Let \(\delta_{d} = \sum_{i}X_{d, i}\). For all component \(d\) such that \(\delta_{d} \geq \frac{1}{2}\), we assign them to the long delay machines \(S'\). To be more precise, we increase their \(X_{d, i}\) variables by a factor of \(1/\delta_{d}\), and set the corresponding \(x_{v, k}, z_{u, v, k}\) to be zero. Since \(\delta_d \geq 1/2\), we have the corresponding constraints.
\begin{align}
  &\sum_{i\in S'} X_{d, i} = 1, &&\forall  d \label{LP:execution_dedup}\\
  &2 D\geq \sum_{d}\frac{X_{d, i}\cdot w(d)}{m_{i}s_{i}}, &&\forall i \label{LP:makespan_Xdi_rounded}
\end{align}

For all other components with \(\delta_{d} < \frac{1}{2}\), set their \(X_{d, i} = 0\). For every job \(v\) in component \(d\), scale its corresponding \(x_{v, k}, y_{v, k}, z_{u, v, k}, C_{v}, C_{u}^{v, k}\) up, by a factor of \(1/(1-\delta_{d})\). In addition, we also replace \(\alpha\) with \(2\alpha\), \(D\) with \(2D\), since \(2\) is an upper bound of \(1/(1 - \delta_{d})\). It is not hard to check that such that all constraints~\labelcref{LP:load,LP:1comm,LP:delay,LP*:load,LP*:precedence,LP*:nonneg,%
  LP*:makespan,LP:makespan,LP:precedence,LP:mincompletion,%
  LP:minexecution,LP:dupload,LP:dupbounds}
holds, and constraint~\labelcref{LP:execution_dedup_simple} degrades to constraint~\labelcref{LP:execution}.  We have thus established that $(C, D, X, x, y, z)$ as defined above satisfies the LP.

\junk{Therefore we have the following lemma.

\begin{lemma}
  After the modifications, the LP is still valid.
\end{lemma}}

Now we need to further the LP variables into a solution. For jobs assigned to \(S\), we use the algorithm of Section~\ref{sec:mdps-no-dup}, and obtain a schedule of length \(\polylog(n) T\). So we only need to round the non-zero \(X_{d,i}\) into an integral solution and get a schedule of connected components (and their jobs) on \(S'\) within time polylog of \(T\), and we actually upper bound it with \(2T + 2D = O(T)\).

We first focus on the load \(w(d)\). Viewing each component as a job, the problem of assigning components to machines is exactly minimizing makespan while scheduling general length jobs on related machines. For this problem, we use a classic result due to Lenstra, Shmoys, and Tardos, restated here for completeness~\cite{lenstra1990approximation}. %(it actually works for unrelated machines, which is a generalization of related machines).

\begin{lemma}[Restatement of Theorem 1 from \cite{lenstra1990approximation}]
  Let \(P = (p_{i, j}) \in \mathbb{Z}_{+}^{m\times n}, (d_{1}, \dots, d_{m})\in \mathbb{Z}_{+}^{m}\), and \(t\in \mathbb{Z}_{+}\).
  Let \(J_{i}(t)\) denote the set of jobs that requre no more than \(t\) time units on machine \(i\), and let \(M_{j}(t)\) denote the set of machines that can process job \(j\) in no more than \(t\) time units. Consider a decision version of scheduling problem where for each machine \(i\) there is a deadline \(d_{i}\) and where we are further constrained to schedule jobs so that each uses processing time at most \(t\); we wish to decide if there is a feasible schedule. If the linear program
  \begin{align*}
    \sum_{i\in M_{j}(t)}x_{ij} &= 1, && j = 1, \dots, n\\
    \sum_{j\in J_{i}(t)}p_{ij}x_{ij} &\leq d_{i}, &&  i = 1, \dots, m\\
    x_{ij} &\geq 0, && \forall j\in J_{i}(t), i = 1, \dots, m
  \end{align*}
  has a feasible solution, then any vertex \(\tilde{x}\) of this polytope can be rounded to a feasible solution \(\bar{x}\) of the integer program
  \begin{align*}
    \sum_{i\in M_{j}(t)}x_{ij} &= 1, && j = 1, \dots, n\\
    \sum_{j\in J_{i}(t)}p_{ij}x_{ij} &\leq d_{i} + t, &&  i = 1, \dots, m\\
    x_{ij} &\in \{0, 1\}, && \forall j\in J_{i}(t), i = 1, \dots, m
  \end{align*}
\end{lemma}

It is not hard to see that if we view components and items, and set \(p_{i,d} = w_{d}/(m_{i}s_{i})\), the constraints are exactly constraints~\labelcref{LP:execution_dedup,LP:makespan_Xdi_rounded}. Therefore we can round them into an integer solution such that,
\begin{equation}
  \sum_{d}\frac{X_{d, i}\cdot w(d)}{m_{i}s_{i}} \leq T + \frac{1}{\delta_{d}}\cdot D, \quad \forall i \label{LP:makespan_Xdi_rounded_integer}
\end{equation}

In other words, for machine \(i\in S'\), the total number of jobs on it is at most \(m_{i}s_{i}(T + 2D)\). Since each DAG has critical path length \(T\), using Graham's list scheduling, we can find a schedule for machine \(i\) in time \(\frac{m_{i}s_{i}(T + 2D)}{m_{i}s_{i}} + T = 2T + 2D\), completing the proof of Lemma~\ref{lem:mdps-symmetric-no-dup} and Theorem~\ref{thm:mdps-symmetric-no-dup}.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> SODA 23/general_proc.tex <==

\section{A Polylogarithmic Approximation Algorithm for \mdps}
\label{sec:approx-mdps}
In this section, we present an asymptotic approximation algorithm for \mdps. Following Lemma~\ref{lem:reduction}, we focus on the setting where $\delayout i = 0$ for all machines $i$. Since there are no out-delays, we use $\delay i$ to denote the in-delay $\delayin i$ of machine $i$.  In Section~\ref{sec:partition}, we first organize the machines according to their size and delay.  Section~\ref{sec:LP} presents a linear programming relaxation, assuming that the machines are organized into groups so that all machines in a group have the same size and delay.   Section~\ref{sec:round} presents a procedure for rounding any fractional solution to the linear program.  Finally, Section~\ref{sec:schedule} presents a combinatorial algorithm that converts an integer solution to the linear program of Section~\ref{sec:LP} to a schedule.  

\subsection{Partitioning machines into groups}
\label{sec:partition}
We first partition machines into groups according to delay and size. Group $\group{\ell,\ell'}$ consists of those machines $i$ such that $\rho_i \le 2^{\ell}$ and $m_i \ge 2^{\ell'}$. \comment{I think we need to give upper/lower bounds on the group parameters -- we don't want ALL machines $i$ with $\rho_i \le 2^{\ell}$}
%For each $\ell, \ell_1, \ell_2$, if there exist groups $\group{\ell, \ell_1}, \group{\ell, \ell_2}$ such that $2^{\ell_1} \ge m \cdot 2^{\ell_2}$, then we eliminate group $\group{\ell,\ell_2}$. 
%We then perform a pairwise compairson of all groups: if, for any $k,k'$, we have $\bar{\rho}_k = \bar{\rho}_{k'}$ and $|\group k| \cdot \bar{m}_k \ge m \cdot  |\group k'| \cdot \bar{m}_{k'}$, we eliminate group $\group{k'}$.
We order the groups arbitrarily $\group 1, \group 2, \ldots, \group K$ and designate the delay and size of all machines in group $\group k$ as $\bar{\rho}_k$ and $\bar m_k$, respectively.  This yields $K = \log \max_k \{ \bar{\rho}_k\} \cdot \log \max_k\{ \bar m_k \}$ groups. Note that if, for any machine $i$, we have $m_i \ge n$, then we can achieve an $\opt$ solution by list scheduling on $i$. So we can assume $\max_k \{ \bar m_k\} \le n$. We can also assume that $\max_k \{\bar{\rho}_k\} \le n$ since, if we ever needed a machine with delay greater than $n$ we could schedule everything on a single machine in less time. Therefore, we have $K \le (\log n)^2$ groups.  
%We define $\rho = \max_i \{\rho_i\}$ and $m = \max_i \{m_i\}$. 
\begin{lemma}
    Increasing the delay of each machine by a factor of 2, and decreasing the size of each machine by a factor of $1/2$, increases the optimal LP solution by a factor of 6.
\label{lem:group_rounding}
\end{lemma}
\begin{proof}
    For each machine $i$, let $k_i$ be such that $i \in \group {k_i}$.  First, we show that increasing the delay of all machines $i$ to $\bar{\rho}_{k_i}$ increases the optimal LP solution by at most a factor of 2. Consider any LP solution $(x^*, y^*, z^*, C^*, D^*)$. Consider the variable assignment $(x^*, y^*,z^*, C', D')$ which is identical to the given assignment except that $C'_v = 2C^*_v$ for all jobs $v$ and $D' = 2 D^*$. It is easy to see that the new assignment is a valid solution with the makespan doubled.
    
    Next, we show that decreasing the size of all machines $i$ to $\bar m_{k_i}$ increases the optimal solution by at most a factor of 3. Given a schedule with completion times $t_v$ for each job $v$. For each machine $i$, we eliminate processors $\ceil{m_i/2}$ to $m_i$ in the worst case. If a job $v$ is executed on an eliminated processor $\floor{m_i/2}+p$ of machine $i$ at time $t$, then we place it on processor $p$ of machine $i$ at time $t^{new}_v = 2t_v + 1$. If a job $v$ is not executed on an eliminated processor, then it is placed on the same processor and executed at time $t^{new}_v = 2t_v$. It is easy to see that the number of processor is halved in the worst case. Suppose that for some pair of jobs $u,v$ we have $t_v - t_u \ge d$. Then $t^{new}_v - t^{new}_u \ge 2t_v - (2t_u+1) = 2(t_v - t_u) - 1 \ge 2d - 1 \ge d$. This shows that all delay and precedence constraints are obeyed. The lemma follows from the fact that the new makespan is at most 3 times the original.
\end{proof}

\subsection{The Linear Program}
\label{sec:LP}
In this section, we design a linear program \LP{a}, parametrized by  $\alpha \ge 1$, for \mdps.  We assume that the machines are organized in groups, where each group $\group k$ is composed of machines that have identical sizes and identical delays.

% Considerations in LP format: All constraints that are replaced in improved result are contiguous. All duplication constraints are contiguous. All constraints that require more space are on the right. All nonstandard constraints are presented first. 
\vspace{-1.5em}
\linearprogram{.58}{.32}{
    &2D \bar{m}_{k} \cdot |\group k| \ge \sum_{v} ( x_{v,k} + y_{v,k} ) &&\forall k 
    \label{LP:load} 
    \\
    &D \ge \bar{\rho}_k \cdot  x_{v,k} &&\forall v,k
    \label{LP:1comm} 
    \\
    &C_v \ge C_u + \bar{\rho}_k \cdot (x_{v,k} - z_{u,v,k} ) &&\forall u,v,k: u \prec v 
    \label{LP:delay} 
    \\
    &\alpha \cdot \bar{\rho}_k \bar m_k \ge \sum_u z_{u,v,k} &&\forall v,k 
    \label{LP*:load}
    \\
    &C^{v,k}_u \ge C^{v,k}_{u'} +  z_{u,v,k} &&\forall u,u',v, k: u' \prec u
    \label{LP*:precedence}
    \\
    &C^{v,k}_u \ge  z_{u,v,k} &&\forall v,u, k 
    \label{LP*:nonneg} 
    \\
    &\alpha \cdot \bar{\rho}_k \ge C^{v,k}_u &&\forall u, v, k
    \label{LP*:makespan}
}{
    &D \ge C_v &&\forall v 
    \label{LP:makespan} 
    \\[.2em]
    &C_v \ge C_u + 1 &&\forall u,v: u \prec v
    \label{LP:precedence} 
    \\[.2em]
    &\sum_{k} x_{v,k} = 1 &&\forall v
    \label{LP:execution}
    \\[.2em]
    &C_v \ge 0 && \forall v
    \label{LP:mincompletion} 
    \\[.2em]
    &x_{v,k} \ge z_{u,v,k} &&\forall u,v, k
    \label{LP:minexecution} 
    \\[.2em]
    &y_{u,k} \ge z_{u,v,k} &&\forall u,v,k
    \label{LP:dupload} 
    \\[.2em]
    &z_{u,v,k} \ge 0 &&\forall u,v,k
    \label{LP:dupbounds} 
}

%\smallskip
\BfPara{Variables} 
$D$ represents the makespan of the schedule. For each job $v$, $C_v$ represents the earliest completion time of $v$. For each job $v$ and group $\group k$, $x_{v,k}$ indicates whether or not job $v$ is first executed on a machine in group $\group k$. For each group $\group k$ and pair of jobs $u,v$ such that $u \prec v$, $z_{u,v,k}$ indicates whether or not $v$ is first executed on a machine in group $\group k$ and the earliest execution of $u$ is less that $\bar{\rho}_k$ time before the execution of $v$. More intuitively, $z_{u,v,k}$ indicates whether there must be a copy of $u$ executed on the same machine that first executes $v$. For each job $v$ and group $\group k$, $y_{v,k}$ indicates whether or not $z_{u,v,k} = 1$ for some $v$; that is, whether or not some copy of $u$ must be placed on group $\group k$. Finally, for each job $v$ and machine group $\group k$, we can think of the variables $\{C^{v,k}_u\}_{u \in V}$ as giving the completion times for a schedule of jobs $u$ such that $z_{u,v.k} = 1$ on a single machine of group $\group k$. Note that constraints~(\ref{LP:makespan}, \ref{LP:mincompletion} - \ref{LP:dupbounds}) guarantee that all variables are non-negative. 


\smallskip
\BfPara{Makespan (\ref{LP:load}, \ref{LP:1comm}, \ref{LP:makespan})}
%The final constraints govern the makespan. The variable $y_{v,k}$ indicates whether or not $v$ is duplicated on group $\group k$.  
% \begin{align}
% &D \ge C_v &&\forall v
% \label{LP:makespan} \\
% &D \ge \bar{\rho}_k \cdot  x_{v,k} &&\forall v,k
% \label{LP:1comm} \\
% &D \cdot |\group k| \cdot \bar{m}_{k} \ge \frac{1}{2} \sum_{v} \Big( x_{v,k} + y_{v,k} \Big) &&\forall k \label{LP:load} \\
% &y_{u,k} \ge z_{u,v,k} &&\forall u,v,k 
% \label{LP:dupload} 
% \end{align}
Constraint~\ref{LP:load} states that the makespan is at least the load on any single group. The factor of 2 is a result of the fact that a single job $v$ may be counted twice on a group $\group k$: once by $x_{v,k}$ and once by $y_{v,k}$. 
Constraint~\ref{LP:1comm} states that we require at least one round of communication to any machine that executes even a single job. This allows us to minimize the additive term in our asymptotic bound.
Constraint~\ref{LP:makespan} states that the makespan is at least the maximum completion time of any job.   


\smallskip
\BfPara{Machine-Dependent Communication delays (\ref{LP:delay})}
%The next set of constraints govern non-uniform communication delays among machines. The variable $x_{v,k}$ indicates whether job $v$ is first executed on a machine in group $\group k$. The variable $z_{u,v,k}$ indicates whether $u \prec v$, $v$ is first executed on a machine in group $k$, and some copy of $u$ is executed on the same machine as $v$ less than $\bar{\rho}_k$ time before the execution of $v$.
%\begin{align}
%&C_v \ge C_u + \bar{\rho}_k \cdot (x_{v,k} - z_{u,v,k} ) &&\forall u \prec v, k 
%\label{LP:delay} \\
%&\sum_{k} x_{v,k} = 1 &&\forall v
%\label{LP:execution} \\
%&x_{v,k} \ge z_{u,v,k} &&\forall u,v, k
%\label{LP:minexecution} \\
%&z_{u,v,k} \ge 0 &&\forall u,v,k
%\label{LP:dupbounds} 
%\end{align}
Constraint~\ref{LP:delay} states that the earliest completion time of $v$ must be at least $\bar{\rho}_k$ after the earliest completion time of any predecessor $u$ if $v$ is first executed on a machine in group $\group k$ and no copy of $u$ is duplicated on the same machine as $v$. % Constraint~\ref{LP:execution} states that every job must be executed on some group.




\smallskip
\BfPara{Duplication (\ref{LP*:load} - \ref{LP*:makespan})}
The next set of constraints govern the amount of duplication allowed for any given job. Fix any job $v$ and group $\group k$, and suppose that $v$ first executes on some machine $i \in \group k$ at time $t$. In order to execute $v$ on $\group k$ at this time, we may need to duplicate some of its predecessors on $i$. Note that only those predecessors that do not complete on any machine by time $t - \bar{\rho}_k$ need to be duplicated on $i$: any predecessors executed on $i$ earlier could have been placed on \textit{any} machine and their results communicated in time. Let $U$ be the set of predecessors of $v$ executed on $i$ after time $t - \bar{\rho}_k$. The duplication constraints ensure that we can schedule $U$ in at most $\bar{\rho}_k$ time on $i$. % The following constraints ensure that this set $U$, by itself, can be scheduled in this amount of time. The variable $C^{v,k}_u$ gives the completion time of $u$ in the schedule of $U$ on $\group k$.
% \begin{align}
% &\alpha \cdot \bar{\rho}_k \ge C^{v,k}_u &&\forall u, v, k
% \label{LP*:makespan}\\
% &\alpha \cdot \bar{\rho}_k \cdot \bar m_k \ge \sum_u z_{u,v,k} &&\forall v,k 
% \label{LP*:load}\\
% &C^{v,k}_u \ge C^{v,k}_{u'} +  z_{u,v,k} &&\forall u,u',v, k: u' \prec u
% \label{LP*:precedence}\\
% &C^{v,k}_u \ge  z_{u,v,k} &&\forall v,u, k 
% \label{LP*:nonneg}
% \end{align}
Intuitively, these constraints capture the load and chain length of the set $U$ which we know, from Graham's list scheduling theorem \cite{graham:schedule}, give tight bounds for no-delay, identical machine scheduling. 
Constraint~\ref{LP*:load} states that the total load that $U$ places on group $\group k$ is no more than $\bar{\rho}_k$.
Constraints~\ref{LP*:precedence} and \ref{LP*:makespan} together guarantee that the maximum chain length in $U$ is at most $\bar{\rho}_k$.  
Constraint~\ref{LP*:nonneg} ensures both that the completion times are non-negative, and that these constraints apply only to those jobs in $U$. 

%\smallskip
%\BfPara{Precedence relations (\ref{LP:precedence})}
%The first set of constraints of \LP{a} govern the precedence relations. Here, the variable $C_v$ represents the completion time of job $v$. 
% \begin{align}
% &C_v \ge C_u + 1 &&\forall u,v,k: u \prec v
% \label{LP:precedence} \\
% &C_v \ge 1 && \forall v
% \label{LP:mincompletion}
% \end{align}
The remaining constraints enforce standard scheduling conditions. 
Constraint~\ref{LP:precedence} states that the completion time of $v$ is at least the completion time of any of its predecessors, and constraint~\ref{LP:execution} ensures that every job is executed on some group. Note that constraints~\ref{LP:execution} and \ref{LP:minexecution} guarantee that $z_{u,v,k} \le 1$ for all $u,v,k$. This is an important feature of the LP, since a large $z$-value could be used to disproportionately reduce the delay between two jobs in constraint~\ref{LP:delay}. %Constraint~\ref{LP:mincompletion} states that no job completes before time 1.




\begin{lemma}{\textbf{(\LP 1 is a valid relaxation)}}
    The minimum value of $D$ for \LP 1 is at most $(\makespan{\sigma} + \delay{\sigma})$, for any schedule $\sigma$.
\label{lem:LP_valid}
\end{lemma}
\begin{proof}
    Consider an arbitrary schedule $\sigma$. We assume the schedule is \textit{minimal} in the sense that a job is executed at most once on any machine and no job is executed on any machine after the result of that job is available to the machine. It is easy to see that, for any non-minimal schedule, there exists a minimal schedule with smaller makespan. We give a solution to the LP in which $D = \makespan{\sigma} + \delay{\sigma}$.
    
    \smallskip
    \BfPara{LP solution} For each job $v$, set $C_v$ to be the earliest completion time of $v$ in $\sigma$. %For each $v$, set $C_v = t_v$. %Set $D = \max_v \{C_v\}$. 
    Set $x_{v,k} = 1$ if $v$ first completes on a machine in group $\group k$ (0 otherwise). For $u,v,k$, set $z_{u,v,k} = 1$ if $u \prec v$, $x_{v,k} = 1$, and $C_v - C_u < \bar{\rho}_k$ (0 otherwise). Set $y_{u,k} = \max_v \{ z_{u,v,k} \}$.
    Fix a job $v$ and group $\group k$. Let $U = \{ u : z_{u,v,k} = 1\}$. If $U = \varnothing$, then set $C^{v,k}_u = 0$ for all $u$. Otherwise, suppose $u \in U$. Then, by assignment of $z_{u,v,k}$, the earliest completion of $v$ is on some machine $i \in \group{k}$. Since the schedule is minimal, we can infer that exactly one copy of $u$ is executed on $i$ as well. Let $t^v_u$ be the completion time of $u$ on $i$. Set $C^{v,k}_u = \bar{\rho}_k - (C_v - t^v_u)$. Now suppose $u \not\in U$. If there is no $u' \in U$ such that $u' \prec u$, then set $C^{v,k}_u = 0$. Otherwise, set $C^{v,k}_u = \max_{u' \prec u} \{C^{v,k}_{u'}\}$. %Set $C^{v,k} = \max_u \{ C^{v,k}_u\}$.
    
    \smallskip
    \BfPara{Feasibility} We now establish that solution defined is feasible. Constraints (\ref{LP:makespan} - \ref{LP:dupbounds}) are easy to verify. We first establish constraints \ref{LP:load} and \ref{LP:1comm}. Consider constraint~\ref{LP:load} for fixed group $\group k$. Both $\sum_v x_{v,k}$ and $\sum_v y_{v,k}$ are upper bound by the total load $L$ on $\group k$. The constraint follows from $D \ge \makespan{\sigma} \ge L / (|\group k| \cdot \bar m_k)$. For fixed $v,k$, constraint~\ref{LP:1comm} holds by assignment of $D$ and definition of $\delay{\sigma}$.
    
    Consider constraint~\ref{LP:delay} for fixed $u,v,k$ where $u \prec v$. Let $X = x_{v,k}$ and let $Z = z_{u,v,k}$. If $(X,Z) = (0,0), (0,1)$, or $(1,1)$ then the constraint follows from constraint \ref{LP:precedence}. Suppose $(X,Z) = (1,0)$. By assignment of $z_{u,v,k}$ we can infer that $C_v - C_u \ge \bar{\rho}_k$, which shows the constraint is satisfied.
    
    To show that constraints (\ref{LP*:load} - \ref{LP*:makespan}) are satisfied, consider fixed $v,k$ and let $U = \{ u: z_{u,v,k} = 1 \}$. If $v$ is not executed on any machine in $\group{k}$ (i.e.\ $x_{v,k} = 0$) then $U = \varnothing$ and the constraints are trivially satisfied by the fact that $C^{v,k}_{u} = 0$ for all $u$. So suppose that $x_{v,k} = 1$.
    \begin{claim}
    The completion times given by $\{C^{v,k}_u\}_{u \in U}$ give a valid schedule of $U$ on any machine in $\group{k}$. 
     \end{claim} 
   \begin{proof}
        Suppose the schedule were not valid for a given machine $i \in \group k$. By assignment of the $C^{v,k}_u$ variables, there are at most $\bar m_k$ jobs scheduled on $i$ in any time step. So the completion times fail to give a schedule only because there is some $u \prec u'$ such that $t^v_u \ge t^v_{u'}$. By the fact that the schedule is minimal, the result of $u$ is not available to $i$ by time $t^v_u$, and so is not available to $i$ by time $t^v_{u'}$. Therefore, the original schedule is not valid, which contradicts our supposition.
    \end{proof}
    
    We proceed to show that (\ref{LP*:load} - \ref{LP*:makespan}) are satisfied using the same fixed $v,k$ and the same definition of $U$.  
    First consider constraint~\ref{LP*:makespan} for fixed $u$. Let $u^* = \arg\max_{u' \in U} \{C^{v,k}_{u'} \}$. By assignment, we have $C^{v,k}_{u^*} \ge C^{v,k}_u$. By definition, we have $C_v = t^v_v$ and $t^v_v > t^v_{u^*}$. Therefore, $C^{v,k}_u \le C^{v,k}_{u^*} = \bar{\rho}_k - (C_v - t^v_{u^*}) = \bar{\rho}_k - (t^v_v - t^v_{u^*}) \le \bar{\rho}_k$, which shows the constraint is satisfied. 
    Consider constraint~\ref{LP*:load}. Let $\widehat{D}$ be the optimal max completion time of scheduling just $U$ on a machine in $\group{k}$. Then
    $\sum_u z_{u,v,k} = |U| \le \widehat{D} \cdot \bar m_{\ell} \le \max_{u \in U} \{C^{v,k}_u\} \cdot \bar m_{\ell}$
    by the claim above. By constraint~\ref{LP*:makespan}, we have that $\max_{u \in U} \{C^{v,k}_u\} \le \bar{\rho}_k$, which entails that the constraint is satisfied.
    Consider constraint~\ref{LP*:precedence} for fixed $u,u'$ such that $u' \prec u$. If $z_{u,v,k} = 0$, then the constraint holds by the fact that $C^{v,k}_u = \max_{\hat u \prec u} \{C^{v,k}_{\hat{u}}\}$. If $z_{u,v,k} = 1$ then the constraint holds by the claim above.
    Finally, for any $u$, constraint~\ref{LP*:nonneg} follows directly from assignment of $C^{v,k}_u$.
\end{proof}

\begin{definition}
    We say that variable assignments $(C,D,x,y,z)$ form an \textit{integer solution} to \LP a if all values of $x,y,z$ are either 0 or 1. 
\end{definition}

\subsection{Deriving an integer solution to the linear program}
\label{sec:round}

Let \LP 1 be defined over groups $\group 1, \group 2, \ldots, \group{K}$. Given a solution $(\hat C, \hat D,\hat x, \hat y, \hat z)$ to \LP 1, we construct an integer solution $(C,D,x,y,z)$ to \LP{2K} as follows. For each $v,k$, set $x_{v,k} = 1$ if $k = \max_{k'}\{\hat x_{v,k'}\}$ (if there is more than one maximizing $k$, arbitrarily select one); set to 0 otherwise. Set $z_{u,v,k} = 1$ if $x_{v,k} = 1$ and $\hat z_{u,v,k} \ge 1/(2K)$; set to 0 otherwise. For all $u,k$, $y_{u,k} = \max_v \{z_{u,v,k}\}$. Set $C_v = 2K \cdot \hat C_v$. Set $C^{v,k}_u =  2K \cdot \hat C^{v,k}_u$. Set $D = 2K \cdot \hat D$. 

\begin{lemma}
    If $(\hat C, \hat D, \hat x, \hat y, \hat z)$ is a valid solution to \LP 1, then  $(C, D, x,y,z)$ is a valid solution to \LP{2K}. 
\label{lem:LPK_solution}
\end{lemma}
\begin{proof}
   \junk{
    We prove that the Constraints~(\ref{LP:precedence}, \ref{LP:mincompletion}, \ref{LP:execution} - \ref{LP:dupbounds}, \ref{LP:makespan}, \ref{LP:dupload}) are easy to verify.
    
    Consider constraint~(\ref{LP:delay}) for fixed $u,v,k$.
    \begin{align*}
        C_v = K \cdot \hat C_v &\ge K(\hat C_u + \bar{\rho}_k (\hat x_{v,k} - \hat z_{u,v,k})) &&\by{supposition} \\
        &= K \hat C_u + \bar{\rho}_k (K \hat x_{v,k} - K \hat z_{u,v,k}) \\
        &\ge C_u + \bar{\rho}_k(x_{v,k} - z_{u,v,k}) &&\by{assignment and (\ref{LP:minexecution})}
    \end{align*}
    }

    %We now show that eliminating the groups with small size machines increases the optimal LP solution by at most a factor of 2, assuming for all $k$ that all machines in $\group k$ have uniform delay $\bar{\rho}_k$ and uniform size $\bar m_k$. \comment{Proof idea: take any LP solution that uses small groups and move all mass onto the largest group of that delay, without changing the completion times of any jobs. The maximum completion time does not increase, and the validity of the solution is maintained. The only thing that changes is the load on the largest group, but this increases at most by a factor of 2.}
By Equation~\ref{LP:execution}, $\sum_{k} \hat x_{v,k}$ is at least 1, so $\max_{k} \{\hat x_{v,k}\}$ is at least $1/K$.  Therefore, $x_{v,k} \le K\hat{x}_{v,k}$ for all $v$ and $k$. By the setting of $C_v$ for all $v$, $C_{u}^{v,k}$ for all $u, v, k$, $y_{v,k}$ for all $v,k$, and $D$, it follows that Equations~\ref{LP:1comm},~\ref{LP*:precedence},~\ref{LP*:makespan}-\ref{LP:dupbounds} of \LP{1} imply the respective equations of \LP{2K}. By definition, $z_{u,v,k} \le 2K \hat z_{u,v,k}$ for any $u,v,k$. So, for any fixed group $\group k$,
\begin{align*}
    4K \hat D \bar m_k \cdot |\group k| &\ge 2K \sum_v (\hat x_{v,k} + \hat y_{v,k}) \ge \sum_v (\hat x_{v,k} + \max_u \{ \hat z_{v,u,k}\}) &&\by{equations \ref{LP:load} and \ref{LP:dupload} of \LP 1} \\
    &\ge 2K \sum_v \Big( \frac{x_{v,k}}{K} + \frac{\max_u \{ z_{v,u,k}\}}{2K} \Big) \ge \sum_v (x_{v,k} + y_{v,k}) &&\by{definition of $y_{v,k}$} 
\end{align*}
which entails Equation~\ref{LP:load} by $D = 2K \hat D$.
Since $z_{u,v,k}$ is 1 only if $x_{v,k}$ is 1, Equation~\ref{LP:minexecution} of \LP{2K} holds.
By definition, $z_{u,v,k} \le 2K \hat{z}_{u,v,k}$, implying that Equations~\ref{LP*:load} and~\ref{LP*:nonneg} of \LP{2K} also hold.  It remains to establish Equation~\ref{LP:delay}.  We consider two cases.  If $\hat{x}_{v,k} < 1/K$, then $x_{v,k} = 0$, so the constraint is trivially true for $v$ and $k$ in \LP{$K$}.  Otherwise, $x_{v,k} - z_{v,k}$ equals $1 - z_{v,k}$, which is 1 only if $x_{v,k} - z_{u,v,k}$ is at least $1/(2K)$.  This establishes Equation~\ref{LP:delay} of \LP{2K} and completes the proof of the lemma. 
\end{proof}

\begin{lemma}
    $D \le 12K (\makespan{\sigma} + \delay{\sigma})$ for any schedule $\sigma$.
\label{lem:LPK_makespan}
\end{lemma}
\begin{proof}
    Lemma~\ref{lem:group_rounding} shows that our grouping of machines does not increase the value of the LP by more than a factor of 6. Therefore, by Lemma~\ref{lem:LP_valid}, $D = 2K \hat D \le 12K (\makespan{\sigma} + \delay{\sigma})$ for any schedule $\sigma$. 
\end{proof}

\subsection{Computing a Schedule given an Integer Solution to the LP}
\label{sec:schedule}

Suppose we are given a partition of $M$ into $K$ groups such that group $\group k$ is composed of identical machines (i.e. identical size and delay). We are also given a valid integer solution $(C,D,x,y,z)$ to \LP a defined over $\group 1, \ldots, \group K$. In this section, we show that we can construct a schedule that achieves a polylogarithmic approximation for \mdps.  

The combinatorial subroutine that constructs the schedule is defined in Algorithm~\ref{alg:scheduler}, which we now describe informally. The subroutine takes as input the integer variable assignments $(C,D,x,y,z)$ and initializes an empty schedule $\sigma$ and global parameter $T$ to 0. For a fixed value of $T$, we check each group $\group k$ to see whether there is some $d \in \mathbb N$ such that $T = d \bar{\rho}_k$. If so, we define $V_{k,d}$ to be the set of jobs $v$ such that $x_{v,k} = 1$ and $T \le C_v < T + \bar{\rho}_k$. We define $U_{v,k}$ to be the set of jobs $u$ such that, for some job $v \in V_{k,d}$, we have $u \prec v$ and $T \le C_u \le t + \bar{\rho}_k$. We then run Identical Machine, Uniform Delay Scheduling on jobs $V_{k,d} \cup U_{k,d}$ using machines in $\group k$ (see Appendix~\ref{sec:uniform}) and append the resulting schedule to $\sigma$. Once all groups $\group k$ have been checked, we increment $T$ and repeat until all jobs are scheduled. The structure of the schedule produced by Algorithm~\ref{alg:scheduler} is depicted in Figure~\ref{fig:schedule_structure}

\begin{algorithm}
\setstretch{1.25}
%\KwData{partially ordered jobs $V$, machines $M$ with associated size and in-delay}
%\KwResult{schedule $\sigma: V \times M \to \mathbb R$}
\KwInit{$\forall v,i, \ \sigma(v,i) \gets \bot;\ T \gets 0$}
\While{$T \le \max_v\{C_v\}$}{
    \ForAll{groups $\group k$}{
        \If{for some integer $d$, $T = d \bar{\rho}_k$}{
            $V_{k,d} \gets \{v: x_{v,k} = 1$ and $T \le C_v < T+ \bar{\rho}_k \} $\;
            $U_{k,d} \gets \{u : \exists v \in V_{k,d},\  u \prec v$ and $T \le C_u < T + \bar{\rho}_k \}$\;
            $\sigma' \gets $ Identical Machine, Uniform Delay Scheduling on $(V_{k,d} \cup U_{k,d}, \group{k})$\;
            $\forall v,i,\ $ if $\sigma'(v,i) \ne \bot$ then $\sigma(v,i) \gets \sigma'(v,i) + \max_{u,j} \{\sigma(u,j)\}$\;
        }
    }
    $T \gets T + 1$\;
}
\caption{Multiprocessor In-Delay Scheduling with Duplication}
\label{alg:scheduler}
\end{algorithm}


The following lemma is proved in Appendix~\ref{sec:uniform}.
\begin{lemma}
    Let $U$ be a set of jobs such that for any $v \in U$ the number of predecessors of $v$ in $U$ (i.e., $|\{ u \prec v\} \cap U|$) is at most $\alpha \bar{\rho}_k \bar m_k$, and the longest chain in $U$ has length at most $\alpha \bar{\rho}_k$. Then given input the set $U$ of jobs and the set $\group k$ of identical machines, Identical Machine, Uniform Delay Scheduling produces, in polynomial time, a valid schedule with makespan less than $3\log(\alpha \bar{\rho}_k \bar m_k)\alpha \bar{\rho}_k + \frac{2 \cdot |U|}{|\group k| \bar m_k}$.
\label{lem:uniform}
\end{lemma}

%We partition jobs into \textit{bands} based on the variable assignments $(C,x,z)$. Band $B_{k,d}$ consists of those jobs $v$ such that $x_{v,k} = 1$ and $d \bar{\rho}_k/\alpha \le C_v < (d+1) \bar{\rho}_k/\alpha$. 

\begin{lemma}
    Algorithm~\ref{alg:scheduler} outputs a valid schedule in polynomial time.
\end{lemma}
\begin{proof}
    It is easy to see that the algorithm runs in polynomial time, and Lemma~\ref{lem:uniform} entails that precedence constraints are obeyed on each machine. Consider a fixed $v,k,d$ such that $v \in V_{k,d}$.
    %and let $U =\{u \prec v: C_v - C_u < \bar{\rho}_k\}$. Suppose that $U \subseteq U_{k,d}$. 
    We know that any schedule on $\group k$ requires an initial communication phase of $\bar{\rho}_k$ time. So, by the time Algorithm~\ref{alg:scheduler} executes any job in $V_{k,d}$, every job $u$ such that $C_u < d\bar{\rho}_k$ is available to every machine in group $\group k$. So the only predecessors of $v$ left to execute are those jobs in $U_{k,d}$. Therefore, all communication constraints are satisfied.
    %So it remains only to show that  $U \subseteq U_{k,d}$. It is sufficient to prove that $z_{u,v,k} = 1$ for all $u \in U$, which follows directly from constraint~\ref{LP:delay}. 
\end{proof}



\begin{lemma}
    If $(C,D,x,y,z)$ is a valid solution to \LP a and $D \le \beta(\makespan{\sigma} + \delay{\sigma})$, then Algorithm~\ref{alg:scheduler} outputs a schedule with makespan at most $O(\alpha\beta K \cdot \log (\alpha \rho m) \cdot (\makespan{\sigma} + \delay{\sigma}))$ for any schedule $\sigma$.
\label{lem:integer_approximation}
\end{lemma}
\begin{proof}
    Note that the schedule produced by the algorithm executes jobs on one group at a time. Since there are $K$ groups, we need only to show that the amount of time spent executing jobs on any group is at most $\alpha^c \log \rho \cdot \opt$.
    
    \begin{claim}
    \label{clm:z}
     For any $u,k,d$, if $u$ is in  $U_{k,d}$, then for some $v$ in $V_{k,d}$ we have $z_{u,v,k} = 1$. 
     \end{claim}
     \begin{proof}
     Fix a job $u$.  If $u$ is in $U_{k,d}$, then by the definition of $U_{k,d}$, there exists a job $v$ in $V_{k,d}$ such that $u \prec v$ and $C_u$ is in $[T, T + \bar{\rho}_k)$, where $T = d\bar{\rho}_k$.  By the definition of $V_{k,d}$, $X_{v,k}$ is 1 and $C_v$ is also in $[T, T + \bar{\rho}_k)$.  Therefore, $C_v - C_u < \bar{\rho}_k$.  But by constraint~(\ref{LP:delay}), $C_v \ge C_u + \bar{\rho}_k(1 - z_{u,v,k})$, implying that $z_{u,v,k}$ cannot equal 0.  Since $z_{u,v,k}$ is either 0 or 1, we have $z_{u,v,k} = 1$. 
     \end{proof}
    
    \begin{claim}
    \label{clm:chain}
For any $v,k,d$, if $v \in V_{k,d}$ then $|\{u \prec v: u \in V_{k,d} \cup U_{k,d}\}|$ is at most $\alpha \bar{\rho}_k \bar m_k$ and the longest chain in $U_{k,d}$ has length at most $\alpha \bar{\rho}_k$.
\end{claim}
\begin{proof} 
Fix $v$ and consider any $u$ in $V_{k,d} \cup  U_{k,d}$ such that $u \prec v$.  
By Claim~\ref{clm:z}, $z_{u,v,k} = 1$.  Therefore, $|\{u \prec v: u \in V_{k,d} \cup U_{k,d}\}|$ equals the right-hand side of Equation~\ref{LP*:load}, and hence at most $\alpha \bar{\rho}_k \bar m_k$.  Let $u_1 \prec u_2 \prec \cdots \prec u_\ell$ denote a longest chain in $U_{k,d}$.  By Claim~\ref{clm:z}, $z_{u_i,v,k}$ equals 1 for $1 \le i \le \ell$.  By Equation~\ref{LP*:nonneg}, $C_{u_1}^{v,k} \ge 1$.  By a repeated application of Equation~\ref{LP*:precedence}, we obtain $C_{u_\ell}^{v,k} \le \ell$.  By Equation~\ref{LP*:makespan}, $\ell \le \alpha \bar{\rho}_k$, and hence the longest chain in $U_{k,d}$ has length at most $\alpha \bar{\rho}_k$.
\end{proof}
    
\begin{claim}
\label{clm:D}
For any $k$, $|\bigcup_d V_{k,d} \cup U_{k,d}| \le D \cdot |\group k| \cdot \bar m_k$.
\end{claim} 
\begin{proof} 
Fix a $k$.  For any $v$ in $V_{k,d}$, by the definition of $V_{k,d}$, $x_{v,k}$ equals 1.  Consider any $u$ in $U_{k,d}$.  By Claim~\ref{clm:z}, there exists a $v$ in $V_{k,d}$ such that $z_{u,v,k}$ equals 1; fix such a $v$.  By Equation~\ref{LP:dupload}, $y_{u,k}$ equals 1.  Thus, $|\bigcup_d V_{k,d} \cup U_{k,d}|$ is at least the right-hand side of Equation~\ref{LP:load}, which is at most  $D \cdot |\group k| \cdot \bar m_k$.
\end{proof}

So, by Lemma~\ref{lem:uniform} and Claim~\ref{clm:chain}, the total time spent executing jobs on a single group is upper bounded by
    \begin{align*}
        \sum_d \Big( 3 \log(\alpha \bar{\rho}_k \bar m_k)  \alpha \bar{\rho}_k + \frac{2 \cdot |V_{k,d} \cup U_{k,d}|}{|\group k| \cdot \bar{m}_k} \Big) &= \frac{3D\alpha \bar{\rho}_k \log(\alpha \bar{\rho}_k \bar m_k)}{\bar{\rho}_k}  + \frac{2}{|\group k| \cdot \bar{m}_k} \sum_d |V_{k,d} \cup U_{k,d}| \\
        &\le 3D\alpha  \log(\alpha \bar{\rho}_k \bar m_k)  + \frac{2D \cdot  |\group k| \cdot \bar m_k}{|\group k| \cdot \bar{m}_k}   \\
        &\le 5D\alpha  \log(\alpha \bar{\rho}_k \bar m_k)  \\
    \end{align*}
    where the second line follows by Claim~\ref{clm:D} and the fact that $D / \bar{\rho}_k \ge 1$. Summing over all groups, we get that the total time in the schedule is at most $5KD\alpha \log(\alpha \rho m)$. The lemma follows from the fact that $D \le \beta \cdot \opt$.
\end{proof}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{Figures/schedule.pdf}
    \caption{Structure of the schedule produced by Algorithm~\ref{alg:scheduler}. $\sigma_{k,d}$ denotes a schedule of $V_{k,d}$ on the machines in group $\group k$. The algorithm scans the $\text{LP}_{\alpha}$ solution by increasing time (left to right). At the start of each $V_{k,d}$, the algorithm constructs a schedule of the set and appends it to the existing schedule.}
    \label{fig:schedule_structure}
\end{figure}

\begin{theorem}
    There exists a polynomial time algorithm that produces a schedule with makespan $O(K^3 \log n \cdot (\makespan{\sigma} + \delay{\sigma})$ for any schedule $\sigma$.
\end{theorem}
\begin{proof}
    Follows from Lemmas~\ref{lem:LPK_solution},  \ref{lem:LPK_makespan}, and~\ref{lem:integer_approximation}.
\end{proof}

==> SODA 23/general_relproc.tex <==

\section{A polylogarithmic approximation algorithm for \mdps}
\label{sec:approx-mdps}
In this section, we present an asymptotic approximation algorithm for \mdps. Following Lemma~\ref{lem:reduction}, we focus on the setting where $\delayout i = 0$ for all machines $i$. Since there are no out-delays, we use $\delay i$ to denote the in-delay $\delayin i$ of machine $i$.  In Section~\ref{sec:partition}, we first organize the machines according to their size, speed, and delay.  Section~\ref{sec:LP} presents a linear programming relaxation, assuming that the machines are organized into groups so that all machines in a group have the same size, speed, and delay.   Section~\ref{sec:round} presents a procedure for rounding any fractional solution to the linear program.  Finally, Section~\ref{sec:schedule} presents a combinatorial algorithm that converts an integer solution to the linear program of Section~\ref{sec:LP} to a schedule.  

\subsection{Partitioning machines into groups}
\label{sec:partition}
We first partition machines into groups according to delay, speed, and size. Group $(\ell_1,\ell_2, \ell_3)$ consists of those machines $i$ such that $2^{\ell_1-1} \le \rho_i < 2^{\ell_1}$, $2^{\ell_2} \le m_i \le 2^{\ell_2+ 1}$, and $2^{\ell_3} \le s_i \le 2^{\ell_3+ 1}$. %For each machine $i \in (\ell_1, \ell_2, \ell_3)$ we redefine $\rho_i = 2^{\ell_1}, m_i = 2^{\ell_2}$, and $s_i = 2^{\ell_3}$. 
We define a new set of machines $M'$. For every $i \in M$, if $i \in (\ell_1, \ell_2, \ell_3)$, we define $i' \in M'$ such that $\rho_i = 2^{\ell_1}$, $m_i = 2^{\ell_2}$, and $s_i = 2^{\ell_3}$. For the remainder of the section, we work with the machine set $M'$. This ensures that every group consists of machines with identical delay, speed, and size, which will simplify the exposition of the algorithm and its proofs. Our reduction to identical machine groups is justified in the following lemma. 

\begin{lemma}
    The optimal makespan over the machine set $M'$ is no more than a factor of 12 greater than the optimal solution over $M$. 
\label{lem:group_rounding}
\end{lemma}
\begin{proof}
    Consider any schedule $\sigma$ on the machine set $M$. We first show that increasing the delay of each machine by a factor of 2 increases the makespan of the schedule by at most a factor of 2. Let $\sigma(v,i)$ be the completion time of $v$ on machine $i$ according to $\sigma$ (and undefined if $v$ is not executed on $i$). We define $\sigma'$ such that $\sigma'(v,i) = 2 \cdot \sigma(v,i)$ (undefined if $\sigma(v,i)$ is undefined). It is easy to see that $\sigma'$ maintains the precedence ordering of jobs, and that the time between the executions of any two jobs has been doubled. Therefore, $\sigma'$ is a valid schedule with all communication delays doubled, and with the makespan doubled.
    
    Next, we show that reducing the size of all machines by a factor of 2 increases the makespan by at most a factor of 3. Let $t_v$ be the completion time of $v$ according to $\sigma$. We define $\sigma'$ as follows. For each machine $i$, we arbitrarily order $i$'s processors $1, \ldots, m_i$. If a job $v$ is executed on processor $\floor{m_i/2}+p$ of machine $i$ at time $t$, then we place it on processor $p$ of machine $i$ at time $t^{new}_v = 2t_v + 1$. If a job $v$ is not executed on an eliminated processor, then it is placed on the same processor and executed at time $t^{new}_v = 2t_v$. It is easy to see that the number of $i$'s processors used is at most half. Suppose that for some pair of jobs $u,v$ we have $t_v - t_u \ge d$. Then $t^{new}_v - t^{new}_u \ge 2t_v - (2t_u+1) = 2(t_v - t_u) - 1 \ge 2d - 1 \ge d$. This shows that all delay and precedence constraints are obeyed and the makespan of $\sigma'$ is at most 3 times the original.
    
    Finally, we show that reducing the speed of each machine by a factor of 2 increases the makespan by at most a factor of 2. Again, by setting $\sigma'(v,i) = 2 \cdot \sigma(v,i)$ (where $\sigma(v,i)$ is defined) we see that the time between any two jobs is increased by a factor of 2 and the makespan is increased by a factor of 2. Therefore, if the speed of each machine is halved, the schedule will remain valid. 
\end{proof}

 We order the groups arbitrarily $\group 1, \group 2, \ldots, \group K$ and designate the delay, size, and speed of all machines in group $\group k$ as $\bar{\rho}_k$, $\bar m_k$, and $\bar s_k$, respectively.  This yields $K = \log \max_k \{ \bar{\rho}_k\} \cdot \log \max_k\{ \bar s_k \bar m_k \}$ groups. Note that if, for any machine $i$, we have $s_i \ge n$, then we can construct a schedule with makespan $1 \le \makespan{\sigma} + \delay{\sigma}$, for any $\sigma$, by placing all jobs on $i$. So we can assume $\max_k \{ \bar s_k \} \le n$. Also, suppose $m_i \ge n$ for any $i$. Then, given a schedule $\sigma$, we can construct the exact same schedule on a machine set where $m_i = n$. So we can assume $\max_k \{ \bar m_k \} \le n$. We can also assume that $\max_k \{\bar{\rho}_k\} \le n$ since, if we ever needed a machine with delay greater than $n$ we could schedule everything on a single machine in less time. 
 
 Therefore, in the most general case, we have $K \le (\log n)^3$ groups. Our approximation ratio accrues several factors of $K$, so we draw attention to special cases in which $K$ is reduced. The reasoning above implies that if any one of the parameters are uniform across all machines, then we have $(\log n)^2$ groups, and if any two of the parameters are uniform we have $\log n$ groups. We emphasize in particular the case with $\log n$ groups where all machine sizes and speeds are uniform and the delay is variable across the machines. 


\subsection{The linear program}
\label{sec:LP}
In this section, we design a linear program \LP{a}, parametrized by  $\alpha \ge 1$, for \mdps.  Following Section~\ref{sec:partition}, we assume that the machines are organized in groups, where each group $\group k$ is composed of machines that have identical sizes, speeds, and delays.

% Considerations in LP format: All constraints that are replaced in improved result are contiguous. All duplication constraints are contiguous. All constraints that require more space are on the right. All nonstandard constraints are presented first. 
\vspace{-1.5em}
\linearprogram{.58}{.3}{
    &2D \bar s_k \bar{m}_{k} \cdot |\group k| \ge \sum_{v} ( x_{v,k} + y_{v,k} ) &&\forall k 
    \label{LP:load} 
    \\
    &D \ge \bar{\rho}_k \cdot  x_{v,k} &&\forall v,k
    \label{LP:1comm} 
    \\
    &C_v \ge C_u + \bar{\rho}_k \cdot (x_{v,k} - z_{u,v,k} ) &&\forall u,v,k: u \prec v 
    \label{LP:delay} 
    \\
    &\alpha \cdot \bar s_k \bar{\rho}_k \bar m_k \ge \sum_u z_{u,v,k} &&\forall v,k 
    \label{LP*:load}
    \\
    &C^{v,k}_u \ge C^{v,k}_{u'} +  \frac{z_{u,v,k}}{\bar s_k} &&\forall u,u',v, k: u' \prec u
    \label{LP*:precedence}
    \\
    &\alpha \cdot \bar{\rho}_k \ge C^{v,k}_u &&\forall u, v, k
    \label{LP*:makespan}
    \\
    &C_v \ge C_u + \sum_k \frac{x_{v,k}}{\bar s_k} &&\forall u,v: u \prec v
    \label{LP:precedence} 
}{
    &D \ge C_v &&\forall v 
    \label{LP:makespan} 
    \\[.35em]
    &\sum_{k} x_{v,k} = 1 &&\forall v
    \label{LP:execution}
    \\[.35em]
    &C_v \ge 0 && \forall v
    \label{LP:mincompletion} 
    \\[.35em]
    &C^{v,k}_u \ge  0 &&\forall v,u, k 
    \label{LP*:nonneg} 
    \\[.35em]
    &x_{v,k} \ge z_{u,v,k} &&\forall u,v, k
    \label{LP:minexecution} 
    \\[.35em]
    &y_{u,k} \ge z_{u,v,k} &&\forall u,v,k
    \label{LP:dupload} 
    \\[.35em]
    &z_{u,v,k} \ge 0 &&\forall u,v,k
    \label{LP:dupbounds} 
}

%\smallskip
\BfPara{Variables} 
$D$ represents the makespan of the schedule. For each job $v$, $C_v$ represents the earliest completion time of $v$. For each job $v$ and group $\group k$, $x_{v,k}$ indicates whether or not $v$ is first executed on a machine in group $\group k$. For each $\group k$ and pair of jobs $u,v$ such that $u \prec v$, $z_{u,v,k}$ indicates whether $v$ is first executed on a machine in group $\group k$ and the earliest execution of $u$ is less that $\bar{\rho}_k$ time before the execution of $v$.  Intuitively, $z_{u,v,k}$ indicates whether there must be a copy of $u$ executed on the same machine that first executes $v$. For each job $v$ and group $\group k$, $y_{v,k}$ indicates whether or not $z_{u,v,k} = 1$ for some $v$; that is, whether or not some copy of $u$ must be placed on group $\group k$. Finally, for each job $v$ and machine group $\group k$, we can think of the variables $\{C^{v,k}_u\}_{u \in V}$ as giving the completion times for a schedule of jobs $u$ such that $z_{u,v.k} = 1$ on a single machine of group $\group k$. Note that constraints~(\ref{LP:makespan}, \ref{LP:mincompletion} - \ref{LP:dupbounds}) guarantee that all variables are non-negative. 


\smallskip
\BfPara{Makespan (\ref{LP:load}, \ref{LP:1comm}, \ref{LP:makespan})}
%The final constraints govern the makespan. The variable $y_{v,k}$ indicates whether or not $v$ is duplicated on group $\group k$.  
% \begin{align}
% &D \ge C_v &&\forall v
% \label{LP:makespan} \\
% &D \ge \bar{\rho}_k \cdot  x_{v,k} &&\forall v,k
% \label{LP:1comm} \\
% &D \cdot |\group k| \cdot \bar{m}_{k} \ge \frac{1}{2} \sum_{v} \Big( x_{v,k} + y_{v,k} \Big) &&\forall k \label{LP:load} \\
% &y_{u,k} \ge z_{u,v,k} &&\forall u,v,k 
% \label{LP:dupload} 
% \end{align}
Constraint~\labelcref{LP:load} states that the makespan is at least the load on any single group. The factor of 2 is a result of the fact that a single job $v$ may be counted twice on a group $\group k$: once by $x_{v,k}$ and once by $y_{v,k}$.
Constraint~\labelcref{LP:1comm} states that we require at least one round of communication to any machine that executes even a single job. This allows us to minimize the additive term in our asymptotic bound.
Constraint~\labelcref{LP:makespan} states that the makespan is at least the maximum completion time of any job.


\smallskip
\BfPara{Machine-Dependent Communication delays (\ref{LP:delay})}
%The next set of constraints govern non-uniform communication delays among machines. The variable $x_{v,k}$ indicates whether job $v$ is first executed on a machine in group $\group k$. The variable $z_{u,v,k}$ indicates whether $u \prec v$, $v$ is first executed on a machine in group $k$, and some copy of $u$ is executed on the same machine as $v$ less than $\bar{\rho}_k$ time before the execution of $v$.
%\begin{align}
%&C_v \ge C_u + \bar{\rho}_k \cdot (x_{v,k} - z_{u,v,k} ) &&\forall u \prec v, k 
%\label{LP:delay} \\
%&\sum_{k} x_{v,k} = 1 &&\forall v
%\label{LP:execution} \\
%&x_{v,k} \ge z_{u,v,k} &&\forall u,v, k
%\label{LP:minexecution} \\
%&z_{u,v,k} \ge 0 &&\forall u,v,k
%\label{LP:dupbounds} 
%\end{align}
Constraint~\labelcref{LP:delay} states that the earliest completion time of $v$ must be at least $\bar{\rho}_k$ after the earliest completion time of any predecessor $u$ if $v$ is first executed on a machine in group $\group k$ and no copy of $u$ is duplicated on the same machine as $v$. % Constraint~\ref{LP:execution} states that every job must be executed on some group.




\smallskip
\BfPara{Duplication (\ref{LP*:load} - \ref{LP*:makespan})}
This set of constraints governs the amount of duplication allowed for any given job. Fix any job $v$ and group $\group k$, and suppose that $v$ first executes on some machine $i \in \group k$ at time $t$. In order to execute $v$ on $i$ at this time, we may need to duplicate some of its predecessors. Note that only those predecessors that do not complete on any machine by time $t - \bar{\rho}_k$ need to be duplicated on $i$: any predecessors executed earlier are available to $i$ by time $t$, regardless of where they are executed. Let $U$ be the set of predecessors of $v$ executed on $i$ after time $t - \bar{\rho}_k$. The duplication constraints ensure that we can schedule $U$ in at most $\bar{\rho}_k$ time on $i$. % The following constraints ensure that this set $U$, by itself, can be scheduled in this amount of time. The variable $C^{v,k}_u$ gives the completion time of $u$ in the schedule of $U$ on $\group k$.
% \begin{align}
% &\alpha \cdot \bar{\rho}_k \ge C^{v,k}_u &&\forall u, v, k
% \label{LP*:makespan}\\
% &\alpha \cdot \bar{\rho}_k \cdot \bar m_k \ge \sum_u z_{u,v,k} &&\forall v,k 
% \label{LP*:load}\\
% &C^{v,k}_u \ge C^{v,k}_{u'} +  z_{u,v,k} &&\forall u,u',v, k: u' \prec u
% \label{LP*:precedence}\\
% &C^{v,k}_u \ge  z_{u,v,k} &&\forall v,u, k 
% \label{LP*:nonneg}
% \end{align}
Intuitively, these constraints capture the load and chain length of the set $U$, via Graham's list scheduling theorem \cite{graham:schedule}, give tight bounds for no-delay, uniform machine scheduling. 
Constraint~\labelcref{LP*:load} states that the total load that $U$ places on group $\group k$ is no more than $\bar{\rho}_k$.
Constraints~\labelcref{LP*:precedence,LP*:makespan} together guarantee that the maximum chain length in $U$ is at most $\bar{\rho}_k$.
%Constraint~\ref{LP*:nonneg} ensures both that the completion times are non-negative, and that these constraints apply only to those jobs in $U$. 

%\smallskip
%\BfPara{Precedence relations (\ref{LP:precedence})}
%The first set of constraints of \LP{a} govern the precedence relations. Here, the variable $C_v$ represents the completion time of job $v$. 
% \begin{align}
% &C_v \ge C_u + 1 &&\forall u,v,k: u \prec v
% \label{LP:precedence} \\
% &C_v \ge 1 && \forall v
% \label{LP:mincompletion}
% \end{align}
The remaining constraints enforce standard scheduling conditions. 
Constraint~\labelcref{LP:precedence} states that the completion time of $v$ is at least the completion time of any of its predecessors, and constraint~\labelcref{LP:execution} ensures that every job is executed on some group.  Constraints~\labelcref{LP:execution,LP:minexecution} guarantee that $z_{u,v,k} \le 1$ for all $u,v,k$. This is an important feature of the LP, since a large $z$-value could be used to disproportionately reduce the delay between two jobs in constraint~\labelcref{LP:delay}. %Constraint~\ref{LP:mincompletion} states that no job completes before time 1.




\begin{lemma}{\textbf{(\LP 1 is a valid relaxation)}}
    The minimum of $D$ for \LP 1 is $\le (\makespan{\sigma} + \delay{\sigma})$, for any schedule $\sigma$.
\label{lem:LP_valid}
\end{lemma}
\begin{proof}
    Consider an arbitrary schedule $\sigma$. We assume the schedule is \textit{minimal} in the sense that a job is executed at most once on any machine and no job is executed on any machine after the result of that job is available to the machine. It is easy to see that if $\sigma$ is not minimal, there exists a minimal schedule $\sigma'$ such that $\makespan{\sigma'} \le \makespan{\sigma}$. We give a solution to the LP in which $D = \makespan{\sigma} + \delay{\sigma}$.
    
    \smallskip
    \BfPara{LP solution} For each job $v$, set $C_v$ to be the earliest completion time of $v$ in $\sigma$. %For each $v$, set $C_v = t_v$. %Set $D = \max_v \{C_v\}$. 
    Set $x_{v,k} = 1$ if $v$ first completes on a machine in group $\group k$ (0 otherwise). For $u,v,k$, set $z_{u,v,k} = 1$ if $u \prec v$, $x_{v,k} = 1$, and $C_v - C_u < \bar{\rho}_k$ (0 otherwise). Set $y_{u,k} = \max_v \{ z_{u,v,k} \}$.
    Fix a job $v$ and group $\group k$. Let $U = \{ u : z_{u,v,k} = 1\}$. If $U = \varnothing$, then set $C^{v,k}_u = 0$ for all $u$. Otherwise, suppose $u \in U$. Then, by assignment of $z_{u,v,k}$, the earliest completion of $v$ is on some machine $i \in \group{k}$. Since the schedule is minimal, we can infer that exactly one copy of $u$ is executed on $i$ as well. Let $t^v_u$ be the completion time of $u$ on $i$. Set $C^{v,k}_u = \bar{\rho}_k - (C_v - t^v_u)$. Now suppose $u \not\in U$. If there is no $u' \in U$ such that $u' \prec u$, then set $C^{v,k}_u = 0$. Otherwise, set $C^{v,k}_u = \max_{u' \prec u} \{C^{v,k}_{u'}\}$. %Set $C^{v,k} = \max_u \{ C^{v,k}_u\}$.
    
    \smallskip
    \BfPara{Feasibility} We now establish that the solution defined is feasible. Constraints (\ref{LP:precedence} - \ref{LP:dupbounds}) are easy to verify. We first establish constraints~\labelcref{LP:load,LP:1comm}. Consider constraint~\labelcref{LP:load} for fixed group $\group k$. Both $\sum_v x_{v,k}$ and $\sum_v y_{v,k}$ are upper bound by the total load $L$ on $\group k$. The constraint follows from $D \ge \makespan{\sigma} \ge L / (|\group k| \cdot \bar s_k \bar m_k)$. For fixed $v,k$, constraint~\labelcref{LP:1comm} holds by assignment of $D$ and definition of $\delay{\sigma}$.
    
    Consider constraint~\labelcref{LP:delay} for fixed $u,v,k$ where $u \prec v$. Let $X = x_{v,k}$ and let $Z = z_{u,v,k}$. If $(X,Z) = (0,0), (0,1)$, or $(1,1)$ then the constraint follows from constraint~\labelcref{LP:precedence}. Suppose $(X,Z) = (1,0)$. By assignment of $z_{u,v,k}$ we can infer that $C_v - C_u \ge \bar{\rho}_k$, which shows the constraint is satisfied.
    
    To show that constraints (\ref{LP*:load} - \ref{LP*:makespan}) are satisfied, consider fixed $v,k$ and let $U = \{ u: z_{u,v,k} = 1 \}$. If $v$ is not executed on any machine in $\group{k}$ (i.e.\ $x_{v,k} = 0$) then $U = \varnothing$ and the constraints are trivially satisfied by the fact that $C^{v,k}_{u} = 0$ for all $u$. So suppose that $x_{v,k} = 1$.
    \begin{claim}
    The completion times given by $\{C^{v,k}_u\}_{u \in U}$ give a valid schedule of $U$ on any machine in $\group{k}$. 
     \end{claim} 
   \begin{proof}
        Suppose the schedule were not valid for a given machine $i \in \group k$. By assignment of the $C^{v,k}_u$ variables, there are at most $\bar m_k$ jobs scheduled on $i$ in any time step. So the completion times fail to give a schedule only because there is some $u \prec u'$ such that $t^v_u \ge t^v_{u'}$. By the fact that the schedule is minimal, the result of $u$ is not available to $i$ by time $t^v_u$, and so is not available to $i$ by time $t^v_{u'}$. Therefore, the original schedule is not valid, which contradicts our supposition.
    \end{proof}
    
    We proceed to show that (\ref{LP*:load} - \ref{LP*:makespan}) are satisfied using the same fixed $v,k$ and the same definition of $U$.  
    First consider constraint~\labelcref{LP*:makespan} for fixed $u$. Let $u^* = \arg\max_{u' \in U} \{C^{v,k}_{u'} \}$. By assignment, we have $C^{v,k}_{u^*} \ge C^{v,k}_u$. By definition, we have $C_v = t^v_v$ and $t^v_v > t^v_{u^*}$. Therefore, $C^{v,k}_u \le C^{v,k}_{u^*} = \bar{\rho}_k - (C_v - t^v_{u^*}) = \bar{\rho}_k - (t^v_v - t^v_{u^*}) \le \bar{\rho}_k$, which shows the constraint is satisfied.
    Consider constraint~\labelcref{LP*:load}. Let $\widehat{D}$ be the optimal max completion time of scheduling just $U$ on a machine in $\group{k}$. Then
    $\sum_u z_{u,v,k} = |U| \le \widehat{D} \cdot \bar s_k \bar m_k \le \max_{u \in U} \{C^{v,k}_u\} \cdot \bar s_k \bar m_k$
    by the claim above. By constraint~\labelcref{LP*:makespan}, we have that $\max_{u \in U} \{C^{v,k}_u\} \le \bar{\rho}_k$, which entails that the constraint is satisfied.
    Consider constraint~\labelcref{LP*:precedence} for fixed $u,u'$ such that $u' \prec u$. If $z_{u,v,k} = 0$, then the constraint holds by the fact that $C^{v,k}_u = \max_{\hat u \prec u} \{C^{v,k}_{\hat{u}}\}$. If $z_{u,v,k} = 1$ then the constraint holds by the claim above.
    %Finally, for any $u$, constraint~\ref{LP*:nonneg} follows directly from assignment of $C^{v,k}_u$.
\end{proof}

\begin{definition}
    $(C,D,x,y,z)$ is an \emph{integer solution} to \LP a if all values of $x,y,z$ are either 0 or 1. 
\end{definition}

\subsection{Deriving an integer solution to the linear program}
\label{sec:round}

Let \LP 1 be defined over groups $\group 1, \group 2, \ldots, \group{K}$. Given a solution $(\hat C, \hat D,\hat x, \hat y, \hat z)$ to \LP 1, we construct an integer solution $(C,D,x,y,z)$ to \LP{2K} as follows. For each $v,k$, set $x_{v,k} = 1$ if $k = \max_{k'}\{\hat x_{v,k'}\}$ (if there is more than one maximizing $k$, arbitrarily select one); set to 0 otherwise. Set $z_{u,v,k} = 1$ if $x_{v,k} = 1$ and $\hat z_{u,v,k} \ge 1/(2K)$; set to 0 otherwise. For all $u,k$, $y_{u,k} = \max_v \{z_{u,v,k}\}$. Set $C_v = 2K \cdot \hat C_v$. Set $C^{v,k}_u =  2K \cdot \hat C^{v,k}_u$. Set $D = 2K \cdot \hat D$. 

\begin{lemma}
    If $(\hat C, \hat D, \hat x, \hat y, \hat z)$ is a valid solution to \LP 1, then  $(C, D, x,y,z)$ is a valid solution to \LP{2K}. 
\label{lem:LPK_solution}
\end{lemma}
\begin{proof}
    By constraint~\labelcref{LP:execution}, $\sum_{k} \hat x_{v,k}$ is at least 1, so $\max_{k} \{\hat x_{v,k}\}$ is at least $1/K$.  Therefore, $x_{v,k} \le K\hat{x}_{v,k}$ for all $v$ and $k$. Also, $z_{u,v,k} \le 2K \hat z_{u,v,k}$ for any $u,v,k$ by definition. By the setting of $C_v$ for all $v$, $C_{u}^{v,k}$ for all $u, v, k$, $y_{v,k}$ for all $v,k$, and $D$, it follows that constraints~(\ref{LP:1comm},~\ref{LP*:load}-\ref{LP:dupbounds}) of \LP{1} imply the respective constraints of \LP{2K}.
    We first establish constraint~\labelcref{LP:load}. For any fixed group $\group k$,
    \begin{align*}
        4K \hat D \bar m_k \bar s_k \cdot |\group k| &\ge 2K \sum_v (\hat x_{v,k} + \hat y_{v,k}) \ge \sum_v (\hat x_{v,k} + \max_u \{ \hat z_{v,u,k}\}) &&\by{constraints~\labelcref{LP:load,LP:dupload} of \LP 1} \\
        &\ge 2K \sum_v \Big( \frac{x_{v,k}}{K} + \frac{\max_u \{ z_{v,u,k}\}}{2K} \Big) \ge \sum_v (x_{v,k} + y_{v,k}) &&\by{definition of $y_{v,k}$} 
    \end{align*}
    which entails constraint~\labelcref{LP:load} by $D = 2K \hat D$.
   % Since $z_{u,v,k}$ is 1 only if $x_{v,k}$ is 1, constraint~(\ref{LP:minexecution}) of \LP{2K} holds.
    %By definition, $z_{u,v,k} \le 2K \hat{z}_{u,v,k}$, implying that constraints~(\ref{LP*:load}) and~(\ref{LP*:nonneg}) of \LP{2K} also hold.  
    It remains to establish constraint~\labelcref{LP:delay} for fixed $u,v,k$.  We consider two cases.  If $\hat{x}_{v,k} < 1/K$, then $x_{v,k} = 0$, so the constraint is trivially true in \LP{2K}.  Otherwise, $x_{v,k} - z_{u,v,k}$ equals $1 - z_{u,v,k}$, which is 1 only if $x_{v,k} - z_{u,v,k}$ is at least $1/(2K)$.  This establishes constraint~\labelcref{LP:delay} of \LP{2K} and completes the proof of the lemma.
\end{proof}

\begin{lemma}
    $D \le 24 \cdot K (\makespan{\sigma} + \delay{\sigma})$ for any schedule $\sigma$.
\label{lem:LPK_makespan}
\end{lemma}
\begin{proof}
    Lemma~\ref{lem:group_rounding} shows that our grouping of machines does not increase the value of the LP by more than a factor of 12. Therefore, by Lemma~\ref{lem:LP_valid}, $D = 2K \hat D \le 24 \cdot K (\makespan{\sigma} + \delay{\sigma})$ for any schedule $\sigma$. 
\end{proof}

\subsection{Computing a schedule given an integer solution to the LP}
\label{sec:schedule}

Suppose we are given a partition of $M$ into $K$ groups such that group $\group k$ is composed of identical machines (i.e. for all $i,j \in \group k$, $s_i = s_j$, $m_i = m_j$, and $\rho_i = \rho_j$). We are also given a valid integer solution $(C,D,x,y,z)$ to \LP a defined over $\group 1, \ldots, \group K$. In this section, we show that we can construct a schedule that achieves an approximation for \mdps\ in terms of $\alpha$ and $K$. The combinatorial subroutine that constructs the schedule is defined in Algorithm~\ref{alg:scheduler}.

We define the Uniform Delay Precedence-constrained Scheduling (\udps) problem to be identical to $\mdps$\ except that, for all $i,j$, $m_i = m_j$, $s_i = s_j$, and $\rho_i = \rho_j$. In Appendix~\ref{sec:uniform}, we give an algorithm \udps-Solver for \udps.


\begin{algorithm}
\setstretch{1.25}
\KwInit{$\forall v,i, \ \sigma(v,i) \gets \bot;\ T \gets 0$}
\While{$T \le \max_v\{C_v\}$}{
    \ForAll{groups $\group k$}{
        \If{for some integer $d$, $T = d \bar{\rho}_k$}{
            $V_{k,d} \gets \{v: x_{v,k} = 1$ and $T \le C_v < T+ \bar{\rho}_k \} $\;
            $U_{k,d} \gets \{u : \exists v \in V_{k,d},\  u \prec v$ and $T \le C_u < T + \bar{\rho}_k \}$\;
            $\sigma' \gets $ \udps-Solver on $(V_{k,d} \cup U_{k,d}, \group{k})$\;
            $\forall v,i,\ $ if $\sigma'(v,i) \ne \bot$ then $\sigma(v,i) \gets \sigma'(v,i) + \max_{u,j} \{\sigma(u,j)\} +   \bar{\rho}_k$ \label{line:append}\;
        }
    }
    $T \gets T + 1$\;
}
\caption{Multiprocessor In-Delay Scheduling with Duplication}
\label{alg:scheduler}
\end{algorithm}


We now describe Algorithm~\ref{alg:scheduler} informally. The subroutine takes as input the integer variable assignments $(C,D,x,y,z)$ and initializes an empty schedule $\sigma$ and global parameter $T$ to 0. For a fixed value of $T$, we check each group $\group k$ to see whether there is some integer $d$ such that $T = d \bar{\rho}_k$. If so, we define $V_{k,d}$ to be the set of jobs $v$ such that $x_{v,k} = 1$ and $T \le C_v < T + \bar{\rho}_k$. We define $U_{v,k}$ to be the set of jobs $u$ such that, for some job $v \in V_{k,d}$, we have $u \prec v$ and $T \le C_u \le t + \bar{\rho}_k$. We then run \udps-Solver on jobs $V_{k,d} \cup U_{k,d}$ using machines in $\group k$ and append the resulting schedule to $\sigma$. Once all groups $\group k$ have been checked, we increment $T$ and repeat until all jobs are scheduled. The structure of the schedule produced by Algorithm~\ref{alg:scheduler} is depicted in Figure~\ref{fig:schedule_structure}.



\begin{lemma}
    Let $U$ be a set of jobs such that for any $v \in U$ the number of predecessors of $v$ in $U$ (i.e., $|\{ u \prec v\} \cap U|$) is at most $\alpha \bar{\rho}_k \bar m_k \bar s_k$, and the longest chain in $U$ has length at most $\alpha \bar{\rho}_k$. Then given as input the set $U$ of jobs and the set $\group k$ of identical machines, \udps-Solver produces, in polynomial time, a valid schedule with makespan less than $3\log(\alpha \bar{\rho}_k \bar m_k \bar s_k)\alpha \bar{\rho}_k + \frac{2 \cdot |U|}{|\group k| \bar m_k \bar s_k}$.
\label{lem:uniform}
\end{lemma}

For a proof of Lemma~\ref{lem:uniform}, see Appendix~\ref{sec:uniform}.

%We partition jobs into \textit{bands} based on the variable assignments $(C,x,z)$. Band $B_{k,d}$ consists of those jobs $v$ such that $x_{v,k} = 1$ and $d \bar{\rho}_k/\alpha \le C_v < (d+1) \bar{\rho}_k/\alpha$. 

\begin{lemma}
    Algorithm~\ref{alg:scheduler} outputs a valid schedule in polynomial time.
\end{lemma}
\begin{proof}
    It is easy to see that the algorithm runs in polynomial time, and Lemma~\ref{lem:uniform} entails that precedence constraints are obeyed on each machine. Consider a fixed $v,k,d$ such that $v \in V_{k,d}$. By line~\ref{line:append}, we insert a communication phase of length $\bar \rho_k$ before appending any schedule on group $\group k$. %any schedule on $\group k$ requires an initial communication phase of $\bar{\rho}_k$ time. 
    So, by the time Algorithm~\ref{alg:scheduler} executes any job in $V_{k,d}$, every job $u$ such that $C_u < d\bar{\rho}_k$ is available to every machine in group $\group k$. So the only predecessors of $v$ left to execute are those jobs in $U_{k,d}$. Therefore, all communication constraints are satisfied.
\end{proof}



\begin{lemma}
    If $(C,D,x,y,z)$ is a valid solution to \LP a and $D \le \beta(\makespan{\sigma} + \delay{\sigma})$, then Algorithm~\ref{alg:scheduler} outputs a schedule with makespan at most $15\alpha\beta K \cdot \log (\alpha n) \cdot (\makespan{\sigma} + \delay{\sigma})$ for any schedule $\sigma$.
\label{lem:integer_approximation}
\end{lemma}
\begin{proof}
    Fix any schedule $\sigma$. Note that the schedule produced by the algorithm executes jobs on one group at a time. Since there are $K$ groups, we need only to show that the amount of time spent executing jobs on any group is at most $\alpha \beta \log (\alpha n) \cdot (\makespan{\sigma} + \delay{\sigma})$.
    
    \begin{claim}
    \label{clm:z}
    For any $u,k,d$, if $u$ is in  $U_{k,d}$, then for some $v$ in $V_{k,d}$ we have $z_{u,v,k} = 1$. 
    \end{claim}
    \begin{proof}
    Fix a job $u$.  If $u$ is in $U_{k,d}$, then by the definition of $U_{k,d}$, there exists a job $v$ in $V_{k,d}$ such that $u \prec v$ and $C_u$ is in $[T, T + \bar{\rho}_k)$, where $T = d\bar{\rho}_k$.  By the definition of $V_{k,d}$, $x_{v,k}$ is 1 and $C_v$ is also in $[T, T + \bar{\rho}_k)$.  Therefore, $C_v - C_u < \bar{\rho}_k$.  By constraint~\labelcref{LP:delay}, $C_v \ge C_u + \bar{\rho}_k(1 - z_{u,v,k})$, implying that $z_{u,v,k}$ cannot equal 0.  Since $z_{u,v,k}$ is either 0 or 1, we have $z_{u,v,k} = 1$.
    \end{proof}
    
    \begin{claim}
    \label{clm:chain}
    For any $v,k,d$, if $v \in V_{k,d}$ then $|\{u \prec v: u \in V_{k,d} \cup U_{k,d}\}|$ is at most $\alpha \bar{\rho}_k \bar m_k \bar s_k$ and the longest chain in $U_{k,d}$ has length at most $\alpha \bar{\rho}_k \bar s_k$.
    \end{claim}
    \begin{proof} 
    Fix $v$ and consider any $u$ in $V_{k,d} \cup  U_{k,d}$ such that $u \prec v$.  
    By Claim~\ref{clm:z}, $z_{u,v,k} = 1$.  Therefore, $|\{u \prec v: u \in V_{k,d} \cup U_{k,d}\}|$ equals the right-hand side of constraint~\labelcref{LP*:load}, and hence at most $\alpha \bar{\rho}_k \bar m_k \bar s_k$.  Let $u_1 \prec u_2 \prec \cdots \prec u_\ell$ denote a longest chain in $U_{k,d}$.  By Claim~\ref{clm:z}, $z_{u_i,v,k}$ equals 1 for $1 \le i \le \ell$.  By constraint~\labelcref{LP*:nonneg}, $C_{u_1}^{v,k} \ge 0$.  By a repeated application of constraint~\labelcref{LP*:precedence}, we obtain $C_{u_\ell}^{v,k} \le \ell$.  By constraint~\labelcref{LP*:makespan}, $\ell \le \alpha \bar{\rho}_k \bar s_k$, and hence the longest chain in $U_{k,d}$ has length at most $\alpha \bar{\rho}_k \bar s_k$.
    \end{proof}
        
    \begin{claim}
    \label{clm:D}
    For any $k$, $|\bigcup_d V_{k,d} \cup U_{k,d}| \le D \cdot |\group k| \cdot \bar m_k \bar s_k$.
    \end{claim} 
    \begin{proof} 
    Fix a $k$.  For any $v$ in $V_{k,d}$ we have $x_{v,k}=1$ by the definition of $V_{k,d}$.  Consider any $u$ in $U_{k,d}$.  By Claim~\ref{clm:z}, there exists a $v$ in $V_{k,d}$ such that $z_{u,v,k}$ equals 1; fix such a $v$.  By constraint~\labelcref{LP:dupload}, $y_{u,k}$ equals 1.  Thus, $|\bigcup_d V_{k,d} \cup U_{k,d}|$ is at most the right-hand side of constraint~\labelcref{LP:load}, which is at most  $D \cdot |\group k| \cdot \bar m_k \bar s_k$.
    \end{proof}
    
    So, by Lemma~\ref{lem:uniform} and Claim~\ref{clm:chain}, the total time spent executing jobs on a single group is upper bounded by
    \begin{align*}
        \sum_d \Big( 3 \log(\alpha \bar{\rho}_k \bar m_k \bar s_k)  \alpha \bar{\rho}_k + \frac{2 \cdot |V_{k,d} \cup U_{k,d}|}{|\group k| \cdot \bar{m}_k \bar s_k} \Big) &= \frac{3D\alpha \bar{\rho}_k \log(\alpha \bar{\rho}_k \bar m_k \bar s_k)}{\bar{\rho}_k}  + \frac{2\sum_d |V_{k,d} \cup U_{k,d}|}{|\group k| \cdot \bar{m}_k \bar s_k}  \\
        &\le 3D\alpha  \log(\alpha \bar{\rho}_k \bar m_k \bar s_k)  + \frac{2D \cdot  |\group k| \cdot \bar m_k \bar s_k}{|\group k| \cdot \bar{m}_k \bar s_k}   \\
        &\le 5D\alpha  \log(\alpha \bar{\rho}_k \bar m_k \bar s_k)  
    \end{align*}
    where the second line follows by Claim~\ref{clm:D} and the fact that $D / \bar{\rho}_k \ge 1$. Summing over all $k$, the total time in the schedule is at most $5KD\alpha \log(\alpha \rho m)$. The lemma follows from the fact that $D \le \beta \cdot (\makespan{\sigma} + \delay{\sigma})$ and $\bar{\rho}_k \bar m_k \bar s_k \le n^3$.
\end{proof}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{Figures/schedule2.pdf}
    \caption{Structure of the schedule produced by Algorithm~\ref{alg:scheduler}. $\sigma_{k,d}$ denotes a schedule of $V_{k,d}$ on the machines in group $\group k$. The algorithm scans the $\text{LP}_{\alpha}$ solution by increasing time (left to right). At the start of each $V_{k,d}$, the algorithm constructs a schedule of the set and appends it to the existing schedule.}
    \label{fig:schedule_structure}
\end{figure}

\begin{theorem}
    There exists a polynomial time algorithm that produces a schedule with makespan $O(K^3 \log n \cdot (\makespan{\sigma} + \delay{\sigma})$ for any schedule $\sigma$.
\end{theorem}
\begin{proof}
    Lemma~\ref{lem:LPK_solution} entails that $(C,D,x,y,z)$ is a valid solution to \LP{2K}. Lemma~\ref{lem:LPK_makespan} entails that $D \le 24 \cdot K(\makespan{\sigma} + \delay{\sigma})$. With $\alpha = 2K$ and $\beta = 24K$,  Lemma~\ref{lem:integer_approximation}  entails that the makespan of our schedule is at most $15K \cdot 2K \cdot 24K \cdot \log(2Kn) \cdot (\makespan{\sigma} + \delay{\sigma})$.
\end{proof}

For the most general case with variable delays, sizes, and speeds, we have $K = (\log n)^3$ groups, yielding an $O((\log n)^{10} \cdot (\makespan{\sigma} + \delay{\sigma}))$ approximation for any schedule $\sigma$. For special cases in which any one parameter is uniform across all machines, we have $K = (\log n)^2$ groups, yielding an $O((\log n)^{7} \cdot (\makespan{\sigma} + \delay{\sigma}))$ approximation for any schedule $\sigma$. For special cases in which any two parameters are uniform across all machines, we have $K = (\log n)$ groups, yielding an $O((\log n)^{4} \cdot (\makespan{\sigma} + \delay{\sigma}))$ approximation for any schedule $\sigma$. %In this last case, a model of particular interest is that in which all machines have uniform (or unit) speed and size, and the in- and out-delays may vary. 

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> SODA 23/improve.tex <==

\section{Improved Bounds with Uniform Total Delay}

In this section, we provide a proof of the following theorem.

\begin{theorem}
Suppose that either the number of processors or total delays are uniform across all machines. There exists a polynomial time algorithm that produces a schedule with makespan at most $O((\log n)^{2} \cdot (\makespan{\sigma} + \delay{\sigma}))$ for any schedule $\sigma$. 
\end{theorem}
\begin{proof}
The theorem follows directly from Lemmas~\ref{lem:integer_approximation}, \ref{lem:integer_imp}, and \ref{lem:makespan_imp}.    
\end{proof}


We introduce the following constraints, which use an ordering on the groups.
\begin{align}
    &C_v \ge C_u + \bar{\rho}_k \sum_{k' = 1}^k (  x_{v,k'} - z_{u,v,k'} ) &&\forall u \prec v, k
    \label{LPimp:delay}    \\
    &\alpha \bar{\rho}_k \bar m_k \ge \sum_u \sum_{k'=1}^k z_{u,v,k'} &&\forall v,k 
    \label{LPimp*:load}\\
    &C^{v,k}_u \ge C^{v,k}_{u'} +  \sum_{k'=1}^k z_{u,v,k'} &&\forall u,u',v, k: u' \prec u
    \label{LPimp*:precedence}\\
    &C^{v,k}_u \ge  \sum_{k'=1}^k z_{u,v,k'} &&\forall v,u, k 
    \label{LPimp*:nonneg}\\
    &D \ge \bar{\rho}_k \cdot \sum_{k' = K}^k  x_{v,k'} &&\forall v,k
    \label{LPimp:1comm} 
\end{align}
For a fixed set of groups, we refer to constraints (\ref{LP:load}, \ref{LP*:makespan} - \ref{LPimp:1comm}) as \LPimp a.

\begin{lemma}
    For any $u,v,k$ such that $u \prec v$, if $\sum_{k'=1}^k x_{v,k'} \ge 1/2$ and  $\hat C_v - \hat C_u < \rho/4$ then $\sum_{k' = 1}^k\hat z_{u,v,k'} \ge 1/4$.%
\label{lem:z_lower}
\end{lemma}
\begin{proof}
    Suppose $\hat z_{u,v,k} < 1/4$. Then 
    \begin{align*}
        \hat C_v \ge \hat C_u + \rho \sum_{k' = 1}^k ( \hat x_{v,k} - \hat z_{u,v,k} ) \ge \hat C_u + (\rho /2) - \rho \sum_{k' = 1}^k \hat z_{u,v,k'}  \ge \hat C_u + \rho/4
    \end{align*}
    which contradicts our supposition.
\end{proof}


% \subsection{Uniform Size Machines, Non-Uniform Delays}
% Group machines by length of their delays: all machines $i$ with $2^{(\log n) - (k+1)} \le \rho_i < 2^{(\log n) - k}$ are in group $\Gamma_k$. Let the \textit{capacity} of $\Gamma_k$ be the number of machines in $\Gamma_k$. We find an optimal solution $(\hat C, \hat D, \hat x, \hat y, \hat z)$ to \LPimp 1 defined over groups $\Gamma_k$. We denote the fixed uniform delay as $\rho$. 

% We now define a new sequence of groups, with $\group 1$ as the group with the highest capacity, and $\group{k+1}$ to be the group with highest capacity such that the machines in $\group{k+1}$ have lower delay than the machines in $\group k$. Using the fractional solution, we define integer assignments $(C, D, x,y,z)$ for \LP 4 defined over $\group 1, \ldots, \group K$. $D = 4K \hat D$. For all $v$, $C_v = 4 \hat C_v$. For all $u,v,k$, $C^{v,k}_u = 4 \hat C^{v,k}_u$. For each $v,k$, set $x_{v,k} = 1$ if $k = \min\{k': \sum_{\ell = 1}^{k'} \hat x_{v,\ell} \ge 1/2\}$; set to 0 otherwise. For each $u,v,k$, set $z_{u,v,k} = 1$ if $x_{v,k} = 1$ and $2 \hat C_v - 2 \hat C_u < \rho$; set to 0 otherwise. For all $u,k$, set $y_{u,k} = \max_v \{ z_{u,v,k}\}$. \comment{some ambiguity here about which groups are being used}

\subsection{Non-Uniform In-Delays, Uniform Machine Size}

We denote the uniform machine size as $m$. Group machines by length of delay: all machines $i$ with $2^{\ell-1} \le \rho_i < 2^{\ell}$ are in group $\Gamma_{\ell}$. We find an optimal solution $(\hat C, \hat D, \hat x, \hat y, \hat z)$ of \LPimp 1 defined over these groups. Let $\med(v) = \min \{\ell : \sum_{\ell'=1}^{\ell} \hat x_{v,\ell'} \ge 1/2\}$.

We now define a new series of groups $\group 1, \group 2, \ldots \group K$. Note that we use the variable $\ell$ to range over groups $\Gamma_{\ell}$ and $k$ to range over groups $\group k$. We define $\group 1 = \arg\max_{\Gamma_{\ell}} \{|\Gamma_{\ell}|\}$ and $\group{k+1} = \arg\max_{\Gamma_{\ell} : \ell < \ell'} \{|\Gamma_{\ell}|: \group k = \Gamma_{\ell'} \}$.  Using the fractional solution $(\hat C, \hat D, \hat x, \hat y, \hat z)$, we define integer assignments $(C, D, x,y,z)$ for \LP 4 defined over $\group 1, \ldots, \group K$. $D = 4K \hat D$. For all $v$, $C_v = 4 \hat C_v$. For all $u,v,k$, $C^{v,k}_u = 4 \hat C^{v,k}_u$. For each $v,k$, set $x_{v,k} = 1$ if $k = \arg\max_{k'} \{ |\group{k'}| : \group{k'} = \Gamma_{\ell}$ and $\ell \le \med(v)\}$; set to 0 otherwise.

Fix $v$ and let $k$ be such that $x_{v,k} = 1$. and let $U = \{u : C_v - C_u < \rho_{\med(v)}\}$. We divide $U$ into $\rho_{\med(v)}/\rho_k$ sets $U_1, \ldots, U_{\rho_{\med(v)}/\rho_k}$. $U_b$ is the set of jobs in chains less than length $\rho_k$ in $U$ after sets $U_{\rho_{\med(v)}/\rho_k}, \ldots, U_{b+1}$ have been removed. For each set $b > 1$, we introduce a dummy job $v_b$ such that $U_b \prec v_b \prec U_{b+1}$. We set $x_{v_b,k} = 1$ and $z_{u,v_b,k} = 1$ for all $u \in U_b$. We set $C_{v_b} = C_v - b\rho_k$.

\begin{figure}
    \centering
    \includegraphics[scale=.7]{Figures/imp_vardelay.pdf}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}





\subsection{Non-Uniform Machine Size, Uniform Total Delay}

Group machines by number of processors: all machines $i$ with $2^k \le m_i < 2^{k+1}$ are in the group $\Gamma_k$. Let the \textit{capacity} of group $\Gamma_k$ be the number of machines in the group times $\bar m_k = 2^k$. We find an optimal solution $(\hat C, \hat D, \hat x, \hat y, \hat z)$ to \LPimp 1. We denote the fixed uniform delay as $\rho$. 



We now define a new series of groups $\group 1, \group 2, \ldots \group K$ such that $\group 1 = \max_k \{|\Gamma_k| \cdot \bar m_k\}$ and $\group{k+1} = \max_{k > k'} \{|\Gamma_k| \cdot \bar m_k : \group k = \Gamma_{k'} \}$.  Using the fractional solution, we define integer assignments $(C, D, x,y,z)$ for \LP 4 defined over $\group 1, \ldots, \group K$. $D = 4K \hat D$. For all $v$, $C_v = 4 \hat C_v$. For all $u,v,k$, $C^{v,k}_u = 4 \hat C^{v,k}_u$. For each $v,k$, set $x_{v,k} = 1$ if $k = \min\{k': \sum_{\ell = 1}^{k'} \hat x_{v,\ell} \ge 1/2\}$; set to 0 otherwise. For each $u,v,k$, set $z_{u,v,k} = 1$ if $x_{v,k} = 1$ and $2 \hat C_v - 2 \hat C_u < \rho$; set to 0 otherwise. For all $u,k$, set $y_{u,k} = \max_v \{ z_{u,v,k}\}$. \comment{some ambiguity here about which groups are being used}

\begin{lemma}
    The integer assignments are a valid solution to \LP 4. 
\label{lem:integer_imp}
\end{lemma}
\begin{proof}
    All constraints except (\ref{LP:load}) are easy to verify from Lemma~\ref{lem:z_lower}, our rounding, and the fact that $(\hat C, \hat D, \hat x, \hat y, \hat z)$ is a valid solution to \LPimp 1 defined over groups $\Gamma_1, \Gamma_2, \ldots$. Consider (\ref{LP:load}) for fixed $k$ such that $\group k = \Gamma_{k'}$.
    \begin{align*}
        \frac{1}{2} \sum_v(x_{v,k} + y_{v,k}) &\le \sum_v x_{v,k} \le 2 \sum_v \sum_{\ell = 1}^{k'} \hat x_{v,\ell} = 2  \sum_{\ell = 1}^{k'} \sum_v \hat x_{v,\ell} &&\by{(\ref{LP:minexecution}, \ref{LP:dupbounds}) and rounding}
        \\
        &\le 2 \sum_{\ell = 1}^{k'} 2 \hat D \cdot |\Gamma_{\ell}| \cdot \bar m_{\ell} \le 4 \hat D \sum_{\ell = 1}^{k'} |\group k| \cdot \bar m_{k}  &&\by{(\ref{LP:load}) and def. of $\group k$}
        \\
        &\le 4 K \hat D \bar m_k \cdot |\group k|  = D \bar m_k \cdot |\group k|  &&\by{def. of $D$}
    \end{align*}
    Note that the second line appeals to $(\hat C, \hat D, \hat x, \hat y, \hat z)$ being a valid solution to \LPimp 1 defined over groups $\Gamma_1, \Gamma_2, \ldots,$ with $\alpha = 1$. This demonstrates that (\ref{LP:load}) is satisfied. 
\end{proof}

\begin{lemma}
    $\hat D \le 6 \cdot \opt + \rho$. 
\label{lem:makespan_imp}
\end{lemma}
\begin{proof}
    Note that Lemma~\ref{lem:group_rounding} entails our grouping of machines $\Gamma_1, \ldots \Gamma_K$ raises $\opt$ by at most a factor of 6. \comment{We could get a better constant, but this is good enough. Might be a good reason to break Lemma~\ref{lem:group_rounding} into multiple lemmas.} To prove the lemma, we show that for any schedule defined over identical machine groups $\Gamma_1, \ldots, \Gamma_k$ with makespan $D^*$, there is a corresponding solution to (\ref{LP:precedence}, \ref{LP:mincompletion}, \ref{LP:execution} - \ref{LP:makespan}, \ref{LP:load} - \ref{LPimp:1comm}) with $\alpha = 1$ and $D = D^*$. Our variable assignments are exactly the same as in Lemma~\ref{lem:LP_valid}, which we repeat here for clarity.
    
    Let $t_v$ be the earliest completion time of job $v$ in the schedule. For each $v$, set $C_v = t_v$. Set $D = \max_v \{C_v\}$. Set $x_{v,k} = 1$ if $v$ first completes on a machine in group $\group k$ (0 otherwise). For $u,v,k$, set $z_{u,v,k} = 1$ if $u \prec v$, $x_{v,k} = 1$, and $C_v - C_u < \rho$ (0 otherwise). Set $y_{u,k} = \max_v \{ z_{u,v,k} \}$.
    
    Fix a job $v$ and group $\group k$. Let $U = \{ u : z_{u,v,k} = 1\}$. If $U = \varnothing$, then set $C^{v,k}_u = 0$ for all $u$. Otherwise, suppose $u \in U$. Then the earliest completion time of $v$ is on some machine $i \in \group{k}$ and, since the schedule is minimal, we can infer that exactly one copy of $u$ is executed on $i$ as well. Let $t^v_u$ be the completion time of $u$ on $i$. Set $C^{v,k}_u = \bar{\rho}_k - (C_v - t^v_u)$. Now suppose $u \not\in U$. If there is no $u' \in U$ such that $u' \prec u$, then set $C^{v,k}_u = 0$. Otherwise, set $C^{v,k}_u \max_{u' \prec u} \{C^{v,k}_{u'}\}$.
    
    Since the variable assignments are the same as Lemma~\ref{lem:LP_valid}, we need only to verify that constraints~(\ref{LPimp:delay} - \ref{LPimp:1comm}) are satisfied. (\ref{LPimp:1comm}) is straightforward.
    
    Consider (\ref{LPimp:delay}) for fixed $u,v,k$. Let $X = \sum_{k'=1}^k x_{v,k'}$ and let $Z = \sum_{k'=1}^k z_{u,v,k'}$. If $(X,Z) = (1,1)$, $(0,1)$, or $(0,0)$ then the constraint is satisfied by (\ref{LP:precedence}). So suppose $X = 1$ and $Z = 0$. In this case, we know that $C_v - C_u \ge \rho$ by our assignment, so the constraint is satisfied.
    
    For constraints~(\ref{LPimp*:load} - \ref{LPimp*:nonneg}), we fix values of $v$ and $k$. Let $U= \{ u: \sum_{k'=1}^k z_{u,v,k'} = 1\}$. By our variable assignments, there is exactly one $k^* \le k$ such that $z_{u,v,k^*} = 1$ for any $u \in U$. Using the same reasoning as in Lemma~\ref{lem:LP_valid}, we have that the completion times given by $\{C^{v,k}_u\}_{u \in U}$ form a valid schedule of $U$ on any machine in group $\group{k^*}$. Since $\group{k^*}$ has smaller size (and the same delay) as group $\group k$, we can infer that these completion times also form a valid schedule of $U$ on any machine in $\group k$. From these facts, we can verify that constraints~(\ref{LPimp*:load} - \ref{LPimp*:nonneg}) are satisfied using the same reasoning as in Lemma~\ref{lem:LP_valid}.
    %Consider (\ref{LPimp*:load}). If $U = \varnothing$, then the constraint is trivially satisfied. Otherwise, by our assignment, there is exactly one group $k^* \le k$ such that $z_{u,v,k^*} = 1$ for any $u \in U$. By our ordering of groups, $\bar m_{k^*} \le \bar m_k$, so the constraint is satisfied. 
    %Consider~(\ref{LPimp*:precedence}) for fixed $u,u'$. If $u$ and $u'$ are both in $U$, then the constraint follows directly from the fact that the values $\{C^{v,k}_u\}_{u \in U}$ form a schedule. If $u' \in U$ and $u \not\in U$, then the constraint follows from the fact that $C^{v,k}_{u} = C^{v,k}_u$. Suppose $u' \not\in U$ and $u \in U$. If $u$ has no predacessors, the constraint holds vacuously. If there is some $u^* \in U$ such that $u' \prec u^* \prec u$, then $C^{v,k}_u > C^{v,k}_{u^*} \ge C^{v,k}_{u'}$ by induction. If there is no such $u^*$, then $C^{v,k}$
    %Consider~(\ref{LPimp*:nonneg}) for fixed $u,v,k$.
    
    Finally, constraint~(\ref{LPimp:1comm}) follows directly from the fact that we've introduced an initial communication phase of length $\rho$ at the start of the given schedule.
\end{proof}

==> SODA 23/intro.tex <==
\section{Introduction}
With the increasing scale and complexity of scientific and data-intensive computations, it is often necessary to process workloads with many dependent jobs on a network of heterogeneous computing devices with varying computing capabilities and communication delays.  
%The heterogeneity among devices is reflected in their differing computing capabilities and networking constraints.  
For instance, the training and evaluation of neural network models, which are iterated directed acyclic graphs (DAGs), is often distributed over diverse devices such as CPUs, GPUs, or other specialized hardware. This process, commonly referred to as \emph{device placement}, has gained significant interest~\cite{mirhoseini2017device,mirhoseini:hierPlace,gao2018spotlight,hafeez2021towards}.  Similarly, many scientific workflows are best modeled as DAGs, and the underlying high-performance computing system as a heterogeneous networked distributed system with communication delays~\cite{andrio2019bioexcel,versluis2018analysis,rico-gallego+dml:hpc}. 

Optimization problems associated with scheduling under communication  delays  have  been  studied  extensively, but  provably  good approximation  bounds  are  few  and  several  challenging  open  problems remain~\cite{ahmad+k:schedule,bampis+gk:schedule,darbha+a:schedule,hoogeveen+lv:schedule,LR02,munier+h:schedule,munier1999approximation,palis1996task,papadimitriou1990towards,picouleau1991two,rayward1987uet}.  With a communication delay, scheduling a DAG of uniform size jobs on identical machines is already
NP-hard~\cite{rayward1987uet,picouleau1991two}, and several inapproximability
results are known~\cite{bampis+gk:schedule,hoogeveen+lv:schedule}.
However, the field is still underexplored and scheduling under communication delay was listed as one of the top ten open problems in scheduling surveys~\cite{bansal:survey,schuurman+w:survey}.  While there has been progress on approximation algorithms for the case of uniform communication delays~\cite{LR02,davies2020scheduling,maiti_etal.commdelaydup_FOCS.20,Liu_etal.linear.22}, little is known for more general delay models.

This paper considers the problem of scheduling precedence-constrained jobs on machines connected by a network with \emph{non-uniform} communication delays.  In general, the delay incurred in communication between two machines could vary with the machines as well as with the data being communicated, which in turn may depend on the jobs being excuted on the machines.  For many applications, however, simpler models suffice.  For instance, job-pairwise delays model scenarios where the delay incurred in the communication between two jobs running on two different machines is a function primarily of the two jobs.  This is suitable when the communication is data-intensive.  On the other hand, machine-pairwise delays, where the delay is only a function of the pair of machines, model scenarios where network latency is the dominant cost of communication.  Recent work in~\cite{davies_etal.nonuniform_SODA.22} presents hardness results for the job-pairwise model, providing preliminary evidence that obtaining sub-polynomial approximation factors may be intractable.  

\subsection{Our contributions}


\begin{wrapfigure}{r}{.4\textwidth}
    \centering
    \includegraphics[width=.35\textwidth]{Figures/inout.pdf}
    \caption{Communicating a result from $i$ to $j$ takes $\delayout i + \delayin  j$ time.}
\label{fig:inout}
\vspace{-0.17in}
\end{wrapfigure}
Our central contribution is that for an important class of machine-pairwise delays, which we call \emph{machine-dependent delays}, polylogarithmic approximations are attainable in polynomial time.  Under machine-dependent delays, each machine $i$ has an in-delay $\delayin i$ and out-delay $\delayout i$, and the time taken to communicate a result from $i$ to $j$ is $\delayout i + \delayin j$.  This model, illustrated in Figure~\ref{fig:inout}, is especially suitable for environments where data exchange between jobs occurs via the cloud, an increasingly common mode of operation in modern distributed systems~\cite{liang+k:cloud,wu+lthzlzj:cloud,mahgoub+ysmebc:cloud}; $\delayin i$ and $\delayout i$ represent the cloud download and upload times, respectively, for machine $i$.   Figure~\ref{fig:problem_tree} situates the machine-dependent delay model and other variants we study in this paper within the landscape of communication delay models.

\begin{definition}{{\bf (Machine-Dependent Precedence-constrained Scheduling \mdps)}}
We are given as input a directed
acyclic graph (DAG), which models a set of $n$ unit size jobs with precedence relations among them,
and a set of $m$ machines.  Each machine has a number $m_i$ of processors and a speed $s_i$ at which each processor processes jobs.
For any job $v$, machine $i$, and time $t$, we say that $v$ is \textit{available} to machine $i$ at time $t$ if $v$ is completed on $i$ before time $t$ or on any machine $j$ before time $t - (\delayin i + \delayout j)$. If job $v$ is scheduled at time $t$ on machine $i$, then all of its predecessors must be available to $i$ by time $t$.  For any schedule $\sigma$, let $\makespan{\sigma}$ denote the makespan of $\sigma$, which is the maximum completion time over all jobs, and let $\delay{\sigma}$ denote $\max\{ \delayin  i + \delayout i\}$ over all machines $i$ on which a job is executed in $\sigma$.  The objective of \mdps\ is to construct a schedule that minimizes makespan.
\end{definition}


\junk{ A natural model is that of a metric.  Special cases of interest are hierarchical metrics or star metrics.  We consider an asymmetric generalization of star metrics, which we refer to as machine-dependent delays.   Motivate this class of problems.
Point to Figure~\ref{fig:problem_tree}.  List theorems. Give high level approach, emphasizing simplicity. Maybe introduce via Chudak-Shmoys simplification? We can also talk about how this approach is also simpler than FOCS paper. Using those more complicated techniques, we can achieve better approximations in settings with uniform size clusters.}

\begin{figure}[ht]
    \centering
    \includegraphics[]{Figures/problemtree2.pdf}
    \caption{Selection of scheduling models with communication delays. $a \to b$ indicates that $b$ is a special case of $a$. We prove individual results for Machine Dependent delays and Symmetric Machine Dependent delays. Citations reflect results relevant to approximation algorithms.}
    \label{fig:problem_tree}
\end{figure}

\junk{
\begin{definition}
For any schedule $\sigma$, let $\makespan{\sigma}$ denote the makespan of $\sigma$, and let $\delay{\sigma}$ denote $\max\{ \delayin  i + \delayout i\}$ over all machines $i$ on which a job is executed in $\sigma$.
\end{definition}
}

We present the first approximation algorithms for scheduling under non-uniform communication delays.  In the presence of delays, a natural approach to hide latency and reduce makespan is to duplicate some jobs (for instance, a job that is a predecessor of many other jobs)~\cite{papadimitriou1990towards,ahmad+k:schedule}.  We consider \mdps\ for both schedules that allow duplication (which we assume by default) and those that do not.   Our main result is a polylogarithmic asymptotic approximation for \mdps\ when duplication is allowed.  

\begin{result}[\textbf{Polylogarithmic asymptotic approximation for \mdps}]
There exists a polynomial time algorithm for \mdps\ that produces a schedule with makespan at most $\polylog(n) \cdot (\makespan{\sigma} + \delay{\sigma})$, for any schedule $\sigma$.%
\label{thm:mdps}
\end{result}
We emphasize that if the makespan of any \mdps\ schedule includes the delays incurred in distributing the problem instance and collecting the output of the jobs, then the algorithm of Theorem~\ref{thm:mdps} is, in fact, a \emph{true polylogarithmic approximation} for makespan.  (From a practical standpoint, in order to account for the time incurred to distribute the jobs and collect the results, it is natural to include in the makespan the in- and out-delays of every machine used in the schedule.)

The exact approximation factor in Theorem~\ref{thm:mdps} depends on the non-uniformity of the particular delay model.  For the most general machine-dependent delays model, our proof achieves a $O(\log^{10} n)$ bound.  We obtain improved bounds when any of the three defining machine parameters---size, speed, and delay---are uniform.  In particular, for the special cases where any two of these parameters are uniform (e.g., when all machines have the same size and speed but different delays), we obtain an $O(\log^4 n)$ bound.  We note that despite some uniformity, these special cases can model certain two-level non-uniform network hierarchies with processors at the leaves, zero or low delays at the first level, and high delays at the second level.    

\junk{
The next theorem presents improved bounds for special cases.
\begin{result}[\textbf{Improved asymptotic approximation for \mdps\ when delays or machine sizes are uniform}]
Suppose that either the number of processors or the delays are uniform across all machines. There exists a polynomial time algorithm that produces a schedule with makespan at most $O((\log n)^{2} \cdot (\makespan{\sigma} + \delay{\sigma}))$ for any schedule $\sigma$. 
\end{result}
The analysis is more complicated, uses optimization from \cite{chudak1999approximation}.
}

We next consider the problem of designing schedules for \mdps\ that do not allow duplication, and obtain a polylogarithmic asymptotic approximation via a reduction to scheduling with duplication.  
\begin{result}[\textbf{Polylogarithmic asymptotic approximation for \mdps\ without duplication}]
\label{thm:mdps-no-dup}
There exists a polynomial time algorithm that produces a no-duplication schedule whose makespan is at most $\polylog(n) (\makespan{\sigma} + \delay{\sigma})$ for any no-duplication schedule $\sigma$. 
\end{result}

\junk{
Note that the first three theorems imply approximation algorithms for the model where there is a central processor that commmunicates other machines. This model requires an initial communication \textit{to} all machines that execute jobs, and a final communication phase \textit{from} all machines that execute jobs. In this model, the makespan of any schedule will be at least the $\delayin  i + \delayout i$ if any job is executed on machine $i$.

[Talk about the challenges involved in removing the additive factor.]}
\noindent Our final result is a true polylogarithmic approximation for no-duplication schedules under symmetric delays.  To achieve this result, we present an approximation algorithm to estimate if the makespan of an optimal no-duplication schedule is at least the delay of any given machine; this enables us to identify machines that cannot communicate in the desired schedule.\footnote{We note that the corresponding problem for duplication schedules is a min-max partitioning variant of the Minimum $k$-Union problem and related to the Min-Max Hypergraph $k$-Partitioning problem, both of which have been shown to be Densest-$k$-Subgraph-hard~\cite{chlamtavc2017minimizing,chandrasekaran+c:partition}; this might suggest a similar hardness result for deriving a \emph{true} approximation for \mdps\ with duplication.} %
\begin{result}[\textbf{Polylogarithmic approximation for \mdps\ with symmetric delays and no duplication}]
\label{thm:mdps-symmetric-no-dup}
If $\delayin  i = \delayout i$ for all $i$, then there exists a polynomial time $\polylog(n)$-approximation algorithm for \mdps\ with no duplication.
\end{result}
\junk{For cases where the optimal makespan is at least the max communication, the previous theorem gives an asymptotic approximation. So, in order to prove this theorem, we present a way to check if opt is less than a given value. Note that, for this setting, the previous theorems give asymptotic approximations -- they minimize $\max_{i,t} \{t + \delayout i + \delayin  i:$ some job is executed on $i$ at time $t\}$.}

\subsection{Our techniques}
Our proof of Theorem~\ref{thm:mdps} relies on a framework consisting of a carefully crafted linear programming relaxation and a series of reductions that derive results  for  \mdps\ % machines with non-uniform speeds, sizes, and delays 
from results for uniform machines. % with uniform parameters.  
While each individual component of the framework is simple or builds on prior work, taken together they offer a flexible recipe for designing approximation algorithms for scheduling DAGs on a distributed system of heterogeneous machines with non-uniform delays. Given the hardness conjectures of \cite{davies_etal.nonuniform_SODA.22} for the job-pairwise setting, we find it surprising that a fairly general machine-pairwise model is tractable. % This may provide evidence that duplication is a powerful tool for solving scheduling problems in different delay settings.

The main components of our \mdps\ algorithm of Theorem~\ref{thm:mdps} are outlined in Figure~\ref{fig:framework}.  First, we observe that any instance of \mdps\ can be reduced to an instance of \mdps\ in which all out-delays are 0, meaning that in the new instance delays depend only on the machine receiving the data.  This reduction is helpful in the second component, which uses a standard method to partition the machines into groups of uniform machines, i.e. each machine in a group can be treated as having the same in-delay, speed, and size (to within a constant factor).  The final approximation factor we establish grows as $K^3$, where $K$ is the number of groups and depends on the extent of non-uniformity among the machines.  We bound $K$ by $O(\log^3 n)$ 
in the general case when the speeds, sizes, and delays of machines are non-uniform.  
%We emphasize that while this partitioning of machines is elementary, it does not partition the scheduling problem among the groups: 
We emphasize that, even with the machines partitioned in this way, an optimal schedule must still judiciously distribute jobs among the groups depending on the structure of the DAG and the particular machine parameters.  

The third component of our algorithm solves an LP relaxation for \mdps\ aimed at finding a placement of the jobs (with possible duplication) on the groups.
%, and solves the LP to obtain fractional variable assignments.  
Building on the approach of~\cite{maiti_etal.commdelaydup_FOCS.20}, our LP uses job placement, duplication, and completion time variables, and incorporates non-uniform speeds, sizes, and communication delays.  %One challenge in incorporating the size is the need to upper bound the amount of duplication allowed for a given job.  When placing job $v$ on machine $i$ at time $t$, the number of duplicates necessary to make this placement is equal to the number of $v$'s predecessors executed on other machines after time $t - \delayin{i}$ (assuming out-delays are 0). Therefore, we must be able to schedule the entire set of duplicated predecessors on machine $i$ in at most $\delayin{i}$ time. Effectively, constraining the set of duplicate predecessors for a given job requires modeling a mini-schedule for that set on the machine where the job is placed. Fortunately, Graham's list scheduling theorem gives us simple parameters by which we can bound the length of any schedule for parallel processors. 
One challenge is bounding the amount of duplication allowed within a communication phase of a particular group. To this end, we incorporate constraints that capture the optimal makespan for scheduling the duplicated jobs on uniform machines. % the load and maximum chain length of duplicated jobs, which are sufficient by Graham's list scheduling theorem \cite{graham:schedule}.
This strategy points to the interesting possibility of capturing more complex processor structure, such as might be modelled with a multi-level tree hierarchy.

The fourth component rounds an optimal LP solution to an integer solution by placing each job on the group for which the job's LP mass is maximized.  A benefit of this simple rounding is that it accommodates many different machine properties as long as the number of groups can be kept small.  Finally, we construct a schedule using the integer LP solution. This subroutine divides the set of jobs assigned to each group into phases and constructs a schedule for each phase by invoking a schedule for the uniform machines case, appending each schedule to the existing schedule for the entire instance.


\junk{ This allows us to capture a more general problem with variable delays, and to greatly simplify the proofs required to establish our bounds. It also means that duplication across groups is not required for our approximation guarantees. Our algorithm allows duplication across groups, but this is entirely to simplify the exposition. }



%Our main technical contribution consists in capturing a difficult problem with a sophisticated linear program, as well as a simple rounding scheme that may extend to more general problems.  

%Our second main technical contribution is to simplify and generalize two prior rounding methods for scheduling. The first method is due to Chudak and Shmoys \cite{chudak1999approximation} who, similar to this paper, use group assignment variables in their LP. In order to optimize their results, the authors order their groups by capacity and assign each job to the highest capacity group with higher index than the job's median group. This method is also used in \cite{maiti_etal.commdelaydup_FOCS.20}, and  is the method on which our improved results are based. However, in \cite{chudak1999approximation}, it is easy to verify that the authors lose only a logarithmic factor by simply placing each job on the group that maximizes the mass of the job. Using this idea, we assign jobs to the group on which its LP mass is highest. \comment{delete paragraph except for $\to$}


%The second method is the schedule construction used in Maiti et al \cite{maiti_etal.commdelaydup_FOCS.20}. This subroutine constructs the schedule phase by phase, placing jobs on all available machines and tracking the progress of each group on the set of jobs assigned to it. The proofs of \cite{maiti_etal.commdelaydup_FOCS.20} do not require all machines to be active at all times and, in fact, only assume that a single group is ever executing jobs. We make make this aspect of their algorithm explicit, scheduling subsets of the jobs assigned to each group one at a time and concatenating the schedules of each group. 


\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{Figures/framework2.pdf}
    \caption{Framework for \mdps\ asymptotic approximation}
    \label{fig:framework}
\end{figure}

The proof of Theorem~\ref{thm:mdps-no-dup}, which extends an asympototic polylogarithmic approximation to no-duplication schedules for general machine-dependent delays, follows from the structure of the schedule designed in Theorem~\ref{thm:mdps} and a general reduction in~\cite{maiti_etal.commdelaydup_FOCS.20} from duplication to no-duplication schedules in the uniform delay case.  Avoiding the additive delay penalty of Theorem~\ref{thm:mdps-no-dup} to achieve the true approximation of Theorem~\ref{thm:mdps-symmetric-no-dup} is more difficult. In the symmetric delay setting, we can distinguish those machines whose delay is low enough to communicate with other machines from those machines with high delay. One of the central challenges is then to distribute jobs among the high-delay machines. We overcome this difficulty by revising the LP in the framework of Theorem~\ref{thm:mdps} to partition the jobs among low- and high-delay machines, and rounding the corresponding solutions separately. We note that  the design of no-duplication schedules via a  reduction to duplication schedules incurs a loss in approximation factor of an additional polylogarithmic factor.  While this may not be desirable in a practical implementation, our results demonstrate the flexibility of the approach and highlight its potential for more general delay models.

\subsection{Related work}

\BfPara{Precedence constrained scheduling}
The problem of scheduling precedence-constrained jobs was initiated in the classic work of Graham who gave a constant approximation algorithm for uniform machines~\cite{graham:schedule}.  Jaffe presented an $O(\sqrt m)$ makespan approximation for the case with related machines~\cite{Jaffe_1980}.  This was improved upon by Chudak and Shmoys who gave an $O(\log m)$ approximation~\cite{chudak1999approximation}, then used the work of Hall, Schulz, Shmoys, and Wein~\cite{Hall_1997} and Queyranne and Sviridenko~\cite{Queyranne_2002} to generalize the result to an $O(\log m)$ approximation for weighted completion time. Chekuri and Bender~\cite{chekuri-bender01} proved the same bound as Chudak and Shmoys using a combinatorial algorithm.  In subsequent work, Li improved the approximation factor to $O(\log m/ \log \log m)$~\cite{Li17}.  The problem of scheduling precedence-constrained jobs is hard to approximate even for identical machines, where the constant depends on complexity assumptions~\cite{LenstraK78, Bansal_2009,Svensson_2010}.
Also, Bazzi and Norouzi-Fard \cite{Bazzi_2015} showed a close connection between structural hardness for \(k\)-partite graph and scheduling with precedence constraints.
% proves the problem on identical machines is hard to approximate to within a factor of \(2 - \epsilon\) assuming a slight variant of UGC conjecture, and the author's pose a hypothesis that, if true, implies super constant hardness for related machines.

\smallskip
\BfPara{Precedence constrained scheduling under communication delays}
Scheduling under communication delays has been studied extensively~\cite{rayward1987uet, papadimitriou1990towards, veltman+ll:schedule}. For unit size jobs, identical machines, and unit delay, a ($7/3$)-approximation is given in \cite{munier+h:schedule}, and \cite{hoogeveen+lv:schedule} proves the NP-hardness of achieving better than a $5/4$-approxmation. Other hardness results are given in \cite{bampis+gk:schedule, picouleau1991two, rayward1987uet}. More recently, Davies, Kulkarni, Rothvoss, Tarnawski, and Zhang \cite{davies2020scheduling} give an $O(\log \rho \log m)$ approximation in the identical machine setting using an LP approach based on Sherali-Adams hierarchy, which is extended to include related machines in~\cite{davies_etal.commdelayrelated_SODA.21}. Concurrently, Maiti, Rajaraman, Stalfa, Svitkina, and Vijayaraghavan \cite{maiti_etal.commdelaydup_FOCS.20} provide a polylogarithmic approximation for uniform communication delay with related machines as a reduction from scheduling with duplication. The algorithm of \cite{maiti_etal.commdelaydup_FOCS.20} is combinatorial in the case with identical machines.  

Davies, Kulkarni, Rothvoss, Sandeep, Tarnawski, and Zhang \cite{davies_etal.nonuniform_SODA.22} consider the problem of scheduling precedence-constrained jobs on uniform machine in the presence of non-uniform, job-pairwise communication delays. That is, if $u \prec v$ and $u$ and $v$ are scheduled on different machines, then the time between their executions is at least $\delay{u,v}$. The authors reduce to this problem from Unique-machines Precedence-Constrained Scheduling (\umps) in which there is no communication delay, but for each job there is some particular machine on which that job must be placed. The authors show that \umps\ is hard to approximate to within a logarithmic factor by a straightforward reduction from job-shop scheduling, and conjecture that \umps\ is hard to approximate within a polynomial factor.

\smallskip
\BfPara{Precedence constrained scheduling under communication delays with job duplication}
Using duplication with communication delay first studied by Papadimitriou and Yannakakis~\cite{papadimitriou1990towards}, who give a 2-approximation for DAG scheduling with unbounded processors and fixed delay. Improved bounds for infinite machines are given in \cite{ahmad+k:schedule, darbha+a:schedule, munier+k:schedule, palis1996task}. Approximation algorithms are given by Munier and Hanen \cite{munier1999approximation, munier+h:schedule} for special cases in which the fixed delay is very small or very large, or the DAG restricted to a tree. The first bounds for a bounded number of machines are given by Lepere and Rapine~\cite{LR02} who prove an asymptotic $O(\log \rho/\log \log \rho)$ approximation. Recent work has extended their framework to other settings:  \cite{maiti_etal.commdelaydup_FOCS.20} uses duplication to achieve an $O(\log \rho \log m/ \log \log \rho)$ approximation for a bounded number of related machines, and Liu, Purohit, Svitkina, Vee, and Wang~\cite{Liu_etal.linear.22} improve on the runtime of~\cite{LR02}  to a near linear time algorithm with uniform delay and identical machines.

%\comment{Empirical results. \cite{lokeshwara+etal.petsd.20}}

\subsection{Discussion and open problems}

Our results indicate several directions for further work. First, we conjecture that our results extend easily to the setting with non-uniform job sizes. We believe the only barriers to such a result are the techinical difficulties of tracking the completion times of very large jobs that continue executing long after they are placed on a machine. Also, while our approximation ratios are the first polylogarithmic guarantees for scheduling under non-uniform delays, we have not attempted to optimize logarithmic factors.  There are obvious avenues for small reductions in our ratio, e.g. the technique used in \cite{LR02} to reduce the ratio by a factor of $\log \log \rho$.  Further reduction, however, may require more novel ideas. Additionally, in the setting without duplication, we incur even more logarithmic factors owing to our reduction to scheduling with duplication. These factors may be reduced by using a more direct method, possibly extending the LP-hierarchy style approach taken in \cite{davies2020scheduling, davies_etal.commdelayrelated_SODA.21}.

Aside from improvements to our current results, our techniques suggest possible avenues to solve related non-uniform delay scheduling problems. Our incorporation of parallel processors allows our results to apply to a two-level machine hierarchy, where machines are the leaves and the delay between machines is a function of their lowest common ancestor.  We would like to explore extensions of our framework to constant-depth hierarchies and tree metrics.  More generally, the problem of scheduling under arbitrary machine metric delays remains wide open. 

Finally, we believe there are useful analogs to these machine-dependent delay models in the job-pairwise regime. A job $v$ with in-delay $\delayin{v}$ and out-delay $\delayout{v}$ has the natural interpretation of the data required to execute a job, and the data produced by a job. A job tree hierarchy could model the shared libraries required to execute certain jobs: jobs in different subtrees require different resources to execute, and downloading these additional resources incurs a delay. Given the hardness conjectures of \cite{davies_etal.nonuniform_SODA.22}, alternate delay models such as these may be necessary to achieve provably good bounds.

%$L$-level hierarchy delays. General metric delays. Generalizing no-duplication approximation to directed star metric. 

%Variable speed machines within clusters. Hardness of checking if OPT less than $\rho_{\max}$ with duplication. Reducing approximation ratio. \comment{We could also mention some similar problems under job-pairwise delays: in/out delays, undirected star, etc. Maybe in open problems?}

%\setcounter{theorem}{0}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> SODA 23/model.tex <==
\section{Model and preliminaries}

\BfPara{Jobs and machines}
Let $V$ denote a set of $n$ unit-size jobs, partially-ordered according to $\prec$.  For any jobs $u$ and $v$ such that $u \prec v$, we refer to $u$ as a \emph{predecessor} of $v$.  Let $M$ denote a set of $m$ machines. We associate with each machine $i \in M$,  an integer \emph{size} $m_i \ge 1$ indicating the number of processors in $i$, an integer speed $s_i \ge 1$ for each processor of $i$, integer \emph{in-delay} of $\delayin {i}$, and integer \emph{out-delay} of $\delayout {i}$.  

\smallskip
\BfPara{Schedules}
A schedule $\sigma$ is an assignment of times to job-machine pairs. If $\sigma(v,i) = t$, this indicates that $v$ is executed on machine $i$ at time $t$ (if $v$ is not executed on $i$ then $\sigma(v,i)$ is undefined).  By default, we allow schedules to duplicate jobs; so, for a given job $v$, $\sigma(v,i)$ and $\sigma(v,j)$ may be defined for distinct machines $i$ and $j$.  In a \emph{no-duplication} schedule, for each job $v$ there is \emph{exactly} one machine $i$ such that $\sigma(v,i)$ is defined. Preemption is not allowed. For any job $v$ machine $i$ and time $t$, we say that $v$ is \textit{available} to $i$ at time $t$ if $v$ is executed on $i$ before time $t$ or on any machine $j$ before time $t - (\delayin i + \delayout j)$. If $v$ is scheduled at time $t$ on machine $i$, then all of its predecessors must be available to $i$ by time $t$. The number of jobs that can be executed on any $i$ at any time $t$ is at most $m_i$. The time to process a single job on any machine $i$ is $1/s_i$. 

Given a set of jobs and machines as above, we let \mdps\ denote the problem of determining a schedule that minimizes the \textit{makespan}, which is the maximum completion time of any job in the schedule. 

\smallskip
\BfPara{Reduction to in-delays}
We first show that \mdps\ reduces to the special case of \mdps\ with zero out-delays. 
This allows us to focus on \mdps\ with zero out-delays in the remainder of the paper.

\begin{lemma}
    For any $\alpha \ge 1$, a polynomial-time $\alpha$-approximation algorithm for \mdps\ (resp., \mdps\ without duplication) in which all out-delays are 0 implies a polynomial-time $\alpha$-approximation for \mdps\ (resp., \mdps\ without duplication).
    \label{lem:reduction}
\end{lemma}
\begin{proof}
    Let $\I$ be an instance of \mdps. We prove the lemma by showing the existence of polynomial-time computable functions $f$ and $f_{\I}$ with the following properties:
    \begin{enumerate*}[label={\bf\small(\alph*)}]
        \item $f(\I)$ is an instance of \mdps\ in which all out-delays are 0, \label{red:indelay}
        \item the optimal makespan of $\I$ is at least the optimal makespan of $f(\I)$, and \label{red:opt}
        \item if $\sigma$ is a schedule (resp., no-duplication schedule) of $f(\I)$ then $f_{\I}(\sigma)$ is a schedule of $\I$ (resp., no-duplication) with the same makespan. \label{red:inverse}
    \end{enumerate*}
    The existence of these functions is sufficient to prove the lemma. For a given schedule $\sigma$ and arbitrary job $v$ and machine $i$, we define $t^{\sigma}_{v,i}$ to be the execution time of $v$ on machine $i$ according to $\sigma$.  
    We first define the instance $f(\I)$ in which all out delays are 0. Since there are no out-delays, we use $\rho_i$ to denote the in-delay of an arbitrary machine $i$ in instance $f(\I)$; $\delayin i$ and $\delayout i$, respectively, denote the in- and out-delay of $i$ in $\I$. $f(\I)$ is identical to $\I$ except that, for each machine $i$, the out-delay of $i$ is 0 and the in-delay $\rho_i$ is equal to $\delayin i + \delayout i$. It is easy to see that $f$ is polynomial-time computable and has property \ref{red:indelay}. 
    
    We show that $f$ has property \ref{red:opt}. Consider a schedule $\sigma$ of $\I$. We construct a schedule $\sigma'$ of $f(\I)$ with the same makespan. For any job $v$ and machine $i$, if $v$ is executed on $i$ at time $t$ according to $\sigma$, then $v$ is executed on $i$ at time $t + \delayout i$ in $\sigma'$. It is easy to see that the makespan (the time at which the result of all jobs is available to the central machine) is the same for both $\sigma$ and $\sigma'$. It is also easy to see that the ordering of jobs on a single machine is maintained in $\sigma'$. So we must only show that the communication constraints are satisfied. Consider two jobs $u$ and $v$ such that $u \prec v$, $u$ is executed on $i$ and $v$ is executed on $j \ne i$, and $t^{\sigma}_{v,j} - t^{\sigma}_{u,i} \ge \delayout i + \delayin j$. Then $t^{\sigma'}_{v,j} - t^{\sigma'}_{u,i} = (t^{\sigma}_{v,j} + \delayout j) - (t^{\sigma}_{u,i} + \delayout i) \ge \delayout i + \delayin j + \delayout j - \delayout i = \delayin j + \delayout j = \rho_j$, implying that $\sigma'$ is a valid schedule of $f(\I)$.   Therefore, property \ref{red:opt} holds.   
    
    We now define $f_{\I}$, which uses similar reasoning as above. Consider a schedule $\sigma$ of $f(\I)$. We define $f_{\I}(\sigma)$ to be schedule $\sigma'$, constructed as follows. For any job $v$ and machine $i$, if $v$ is executed on $i$ at time $t$ according to $\sigma$, then $v$ is executed on $i$ at time $t - \delayout i$ according to $\sigma'$. Note that the definition ensures that if $\sigma$ is a no-duplication schedule, then so is $\sigma'$.  Again, it is easy to see that $f_{\I}$ is polynomial-time computable, that the makespan is the same for both schedules, and that precedence constraints are maintained on individual machines. So consider two jobs $u$ and $v$ such that $u \prec v$, $u$ is executed on $i$ and $v$ is executed on $j \ne i$, and $t^{\sigma}_{v,j} - t^{\sigma}_{u,i} \ge \rho_j = \delayin j + \delayout j$. Then $t^{\sigma'}_{v,j} - t^{\sigma'}_{u,i} = (t^{\sigma}_{v,j} - \delayout j) - (t^{\sigma}_{u,i} - \delayout i) \ge \delayin j + \delayout j - \delayout j + \delayout i = \delayin j + \delayout i$, implying that $\sigma'$ is a valid schedule of $\I$.   Therefore, property \ref{red:inverse} holds.  
\end{proof}

%Throughout the paper, when machines are divided into groups of identical machines, we use $\bar{\rho}_k$ and $\bar m_k$ to denote, respectively, the in-delay and size of all machines in the group with index $k$.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> SODA 23/udps.tex <==
\section{Algorithm for Uniform Machines}
\label{sec:uniform}

In this section, we show the existence of an algorithm which achieves provably good bounds for scheduling on uniform machines with fixed communication delay. The algorithm presented here is a generalization of the algorithm in \cite{LR02}, the main difference being our incorporation of parallel processors for each machine. 

Recall that \udps\ is identical to \mdps\ with $\delayout{i} = 0$ for all $i$, and with $\rho_i = \rho_j$, $m_i = m_j$, and $s_i = s_j$ for all $i,j$. We define \udps-Solver as \Cref{alg:uniform}. The algorithm takes as input a set of jobs $U$ and a group $\group k$ of identical machines with delay $\bar{\rho}_k$, speed $\bar s_k$, and size $\bar m_k$. We are guaranteed that the length of the longest chain in $U$ is at most $\alpha \bar{\rho}_k \bar s_k$ and that, for any job $v \in U$, the number of jobs $u \in U$ such that $u \prec v$ is at most $\alpha \bar{\rho}_k \bar m_k \bar s_k$.

\begin{algorithm}
\KwData{set of jobs $U$, set of identical machines $\group k$}
\KwInit{$t \gets 0$\;}
\While{$U \ne \varnothing$}{
    $\forall i \in \group k,\  V_{i,t} \gets \varnothing$ \label{line:Vit_init}\;
    \ForAll{jobs $v \in U$}{
        $U_{v,t} \gets \{u \in U: u \prec v\}$\;
        $U^{\dup}_{v,t} \gets U_{v,t} \cap \{u \in U : u \prec v$ and $\exists i, u \in V_{i,t} \}$\;
        \If{$|U_{v,t}| \ge 2 \cdot |U^{\dup}_{v,t}|$ \label{line:overlap}}{
            $i \gets \arg\min_{j \in \group k} \{ | V_{j,t} | \}$ \label{line:machine}\;
                $V_{i,t} \gets V_{i,t} \cup U_{v,t}$ \label{line:place}\;
        }
    }
    $\forall i \in \group k$, list schedule $V_{i,t}$ on $i$ starting at time $t$\;
    $U \gets U \setminus \big( \bigcup_i V_{i,t} \big)$ \label{line:remove}\;
    $t \gets \bar{\rho}_k + \max\{ t, \max_{v} \{$completion time of $v\}\}$ \label{line:update_t}\;
}
\caption{\udps-Solver}
\label{alg:uniform}
\end{algorithm}

\begin{lemma}
    \Cref{alg:uniform} produces a valid schedule of $U$ on $\group k$ in polynomial time.
\end{lemma} 
\begin{proof}
    For fixed $i,t$, the list scheduling subroutine guarantees that precedence constraints are maintained in placing $V_{i,t}$. So we must only show that precedence and communication constraints are obeyed across different values of $t$. For a fixed value $t^*$, line~\ref{line:remove} entails that all jobs in $\bigcup_i V_{i,t}$ for $t < t^*$ have been removed from $U$. This entails that all precedence constraints are obeyed in scheduling $V_{i,t^*}$. The update at line~\ref{line:update_t} ensure that no jobs are executed for $\bar{\rho}_k$ before scheduling $V_{i,t^*}$. Since there is no communication necessary for scheduling $\bigcup_i V_{i,t^*}$, this entails that communication constraints are obeyed.  
\end{proof}

\begin{lemma}
    For any $t$, $\sum_i |V_{i,t}| \le 2 \cdot |\bigcup_i V_{i,t}|$.
    \label{lem:dup_load}
\end{lemma}
\begin{proof}
    Consider a fixed value of $t$. For any machine $i$, let $V_{i,t,0}$ be the value of $V_{i,t}$ after initialization at line~\ref{line:Vit_init}. Also, for all machines $i$, let $V_{i,t,\ell}$ be the value of $V_{i,t}$ after the $\ell$\textsuperscript{th} time some set $V_{j,t}$ is updated.  We prove the lemma by induction on $\ell$. 
    
    The lemma holds trivially for $\ell = 0$ since $\sum_i |V_{i,t,0}| = |\bigcup_i V_{i,t,0}| = 0$. Suppose the lemma holds up until the $\ell$\textsuperscript{th} update of any $V_{i,t}$, and consider the $(\ell + 1)$\textsuperscript{th} update. Let $U'$ be the set of jobs placed during the update. The condition at line~\ref{line:overlap} entails that at least half the jobs in $U$ are not in $\bigcup_i V_{i,t,\ell}$. Therefore,
    \begin{align*}
        |\bigcup_i V_{i,t,\ell+1}| &= |U \cup \bigcup_i V_{i,t,\ell}| = |U| + |\bigcup_i V_{i,t,\ell}| - |U \cap \bigcup_i V_{i,t,\ell}| \\
        &\ge |U| + |\bigcup_i V_{i,t,\ell}| - \frac{|U|}{2} &&\by{supposition}\\
        &\ge \frac{|U|}{2} + \frac{\sum_i |V_{i,t,\ell}|}{2} \ge \frac{1}{2} \sum_i |V_{i,t,\ell+1}| &&\by{IH} 
    \end{align*}
    This proves the lemma.
\end{proof}

\begin{lemma}
    If $t_1$ and $t_2$ are two consecutive values of $T$, then $t_2 \le t_1 + \frac{2 \cdot |\bigcup_i V_{i,t}|}{|\group k| \cdot \bar m_k \bar s_k} + 3\alpha \bar{\rho}_k$. 
\label{lem:load_balance}
\end{lemma}
\begin{proof}
    Consider a fixed value of $t$. If there are no jobs added to $V_{i,t}$ for any $i$, then $t_2 = t_1 + \bar{\rho}_k$ by line~\ref{line:update_t} and the lemma holds. So suppose that $\max_v\{$completion time of $v\} > t_1$ on execution of line~\ref{line:update_t}. At the execution of this line, suppose the last job completes on machine $i^*$. Then 
    \begin{align*}
        t_2 &= \bar{\rho}_k + t_1 + \max_v\{\text{completion time of } v \text{ on } i^*\} - t_1 &&\by{line~\ref{line:update_t}}\\
        &\le \bar{\rho}_k + t_1 + \frac{|V_{i^*,t}|}{\bar m_k \bar s_k} + (\text{length of longest chain in } U) &&\by{Graham \cite{graham:schedule}} \\
        &\le \bar{\rho}_k + t_1 + \frac{|V_{i^*,t}|}{\bar s_k \bar m_k} + \alpha \bar{\rho}_k &&\by{supposition} \\
        &\le \bar{\rho}_k + t_1 + \min_i \Big\{ \frac{|V_{i,t}|}{\bar m_k \bar s_k} \Big\} + \frac{\alpha \bar{\rho}_k \bar m_k \bar s_k}{\bar m_k \bar s_k} + \alpha \bar{\rho}_k &&\by{supposition and line~\ref{line:machine}} \\
        &\le  t_1 + \frac{\sum_i |V_{i,t}|}{|\group k| \cdot \bar m_k \bar s_k} + \bar{\rho}_k (2 \alpha + 1) \le t_1 + \frac{2 \cdot |\bigcup_i V_{i,t}|}{|\group{k}| \cdot \bar m_k \bar s_k} + \bar{\rho}_k (2\alpha + 1) &&\by{Lemma~\ref{lem:dup_load}}
    \end{align*}
    The appeal to line~\ref{line:machine} invokes the fact that the algorithm always chooses the least loaded machine when placing new jobs. Since every job has a maximum of $\alpha \bar{\rho}_k \bar m_k \bar s_k$ predecessors in $U$, by supposition, the difference $|V_{i,t}| - |V_{j,t}|$ is always maintained to be less than  $\alpha \bar{\rho}_k \bar m_k \bar s_k$, for any $i,j$. This proves the lemma.
\end{proof}

\begin{lemma}%[Restatement of Lemma~\ref{lem:uniform}]
    Let $U$ be a set of jobs such that for any $v \in U$ the number of predecessors of $v$ in $U$ (i.e., $|\{ u \prec v\} \cap U|$) is at most $\alpha \bar{\rho}_k \bar m_k \bar s_k$, and the longest chain in $U$ has length at most $\alpha \bar{\rho}_k$. Then given as input the set $U$ of jobs and the set $\group k$ of identical machines, \udps-Solver produces, in polynomial time, a valid schedule with makespan less than $3\log(\alpha \bar{\rho}_k \bar m_k \bar s_k)\alpha \bar{\rho}_k + \frac{2 \cdot |U|}{|\group k| \bar m_k \bar s_k} + \bar{\rho}_k$.
\label{lem:udps}
\end{lemma}

\begin{proof}
    By the condition of line~\ref{line:overlap}, each time the variable $t$ increments we can infer that all unscheduled jobs have their number of unscheduled predecessors halved. By our supposition, this entails $t$ can be incremented only  $\log(\alpha \bar{\rho}_k \bar m_k \bar s_k)$ times before all jobs are scheduled. Let $t_{\ell}$ be $\ell$\textsuperscript{th} value of $t$, for $\ell = 0, 1, 2, \ldots, \log(\alpha \bar{\rho}_k \bar m_k)$. 
    \begin{claim}
        For any $\ell$, we have  $\displaystyle t_{\ell + 1} \le 3\ell \alpha \bar{\rho}_k +  \frac{2 \cdot |\bigcup_i \bigcup_{\ell' = 0}^{\ell} V_{i,t_{\ell'}}| }{|\group k| \cdot \bar m_k} + \bar{\rho_k}$
    \end{claim}
    \begin{proof}
        We prove the claim by induction on $\ell$. For $\ell = 0$, the claim holds since the inital value of $t$ is $0$. Suppose the claim holds up to $\ell$. Then 
        \begin{align*}
            t_{\ell + 1} &\le t_{\ell} + \frac{2 \cdot |\bigcup_i V_{i,t_{\ell}}|}{|\group k| \cdot \bar m_k} + 3 \alpha \bar{\rho}_k  &&\by{Lemma~\ref{lem:load_balance}}\\
            &\le 3 \ell \alpha \bar{\rho}_k + \frac{2 \cdot |\bigcup_i \bigcup_{\ell' = 1}^{\ell-1} V_{i, t_{\ell'}}|}{|\group k| \cdot \bar m_k} + \frac{2 \cdot |\bigcup_i V_{i,t_{\ell}}|}{|\group k| \cdot \bar m_k} + 3 \alpha \bar{\rho}_k  &&\by{I.H.} \\
            &\le 3 \alpha \bar{\rho}_k(\ell + 1) +  \frac{2 \cdot |\bigcup_i \bigcup_{\ell' = 1}^{\ell} V_{i, t_{\ell'}}|}{|\group k| \cdot \bar m_k} %&&\by{} \bigcup_i V_{i,t_{\ell}} \cap \bigcup_i \bigcup_{\ell' = 1}^{\ell-1} V_{i, t_{\ell'}} = \varnothing 
        \end{align*}
        where the last line follows from the fact that $\bigcup_i V_{i,t_{\ell}}$ and $\bigcup_i \bigcup_{\ell' = 1}^{\ell-1} V_{i, t_{\ell'}}$ have no members in common.
    \end{proof}
    The claim is sufficient to establish the lemma.
\end{proof}

==> STOC 23/machine.tex <==

\section{A polylogarithmic approximation algorithm for machine delays}
\label{sec:approx-mdps}
In this section, we present an asymptotic approximation algorithm for machine delays with unit speed and size machiens. Following Lemma~\ref{lem:reduction}, we focus on the setting where $\delayout i = 0$ for all machines $i$. Since there are no out-delays, we use $\delay i$ to denote the in-delay $\delayin i$ of machine $i$.  In Section~\ref{sec:partition}, we first organize the machines according delay.  Section~\ref{sec:LP} presents a linear programming relaxation, assuming that the machines are organized into groups so that all machines in a group have the same delay.   Section~\ref{sec:round} presents a procedure for rounding any fractional solution to the linear program.  Finally, Section~\ref{sec:schedule} presents a combinatorial algorithm that converts an integer solution to the linear program of Section~\ref{sec:LP} to a schedule.  

\subsection{Partitioning machines into groups}
\label{sec:partition}
In order to simplify the remainder of the paper, we introduce a new set of machines $M'$ with rounded delays. For each $i \in M$, if $2^{k-1} \le \delay i < 2^{k}$, we define $i' \in M$ such that $\delay{i'} = 2^k$. We then partition $M'$ according to machine delays: machine $i \in M'$ is in $\group k$ if $\delay i = 2^k  = \groupdelay k$. For the remainder of the section, we work with the machine set $M'$, ensuring that every group consists of machines with identical delay. This simplifies the exposition of the algorithm and its proofs. Our reduction to identical machine groups is justified in the following lemma.

\begin{lemma}
    The optimal makespan over the machine set $M'$ is no more than $2 \cdot \opt$.  
\label{lem:group_rounding}
\end{lemma}
\begin{proof}
    Consider any schedule $\sigma$ on the machine set $M$. We first show that increasing the delay of each machine by a factor of 2 increases the makespan of the schedule by at most a factor of 2. We define the schedule $\sigma'$ as follows. For every $i,t$, if $(i,t) \in \sigma(v)$, then $(i,2t) \in \sigma'(v)$. It is easy to see that $\sigma'$ maintains the precedence ordering of jobs, and that the time between the executions of any two jobs has been doubled. Therefore, $\sigma'$ is a valid schedule with all communication delays doubled, and with the makespan doubled.
\end{proof}

We can assume that $\max_k \{\groupdelay k\} \le n$ since, if we ever needed a machine with delay greater than $n$ we could schedule everything on a single machine in less time. Therefore we have $K \le \log n$ groups. 
%Our approximation ratio accrues several factors of $K$, so we draw attention to special cases in which $K$ is reduced. The reasoning above implies that if any one of the parameters are uniform across all machines, then we have $(\log n)^2$ groups, and if any two of the parameters are uniform we have $\log n$ groups. We emphasize in particular the case with $\log n$ groups where all machine sizes and speeds are uniform and the delay is variable across the machines. 


\subsection{The linear program}
\label{sec:LP}
In this section, we design a linear program \LP{a}, parametrized by  $\alpha \ge 1$, for machine delays.  Following Section~\ref{sec:partition}, we assume that the machines are organized in groups, where each group $\group k$ is composed of machines that have identical delay.
 
\vspace{-1.5em}
\linearprogram{.58}{.3}{
    &\Calpha \ge C_v &&\forall v 
    \label{LP:makespan} 
    \\
    &\Calpha \cdot |\group k| \ge \sum_{v} y_{v,k} &&\forall k 
    \label{LP:load} 
    \\
    %&D \ge \bar{\rho}_k \cdot  x_{v,k} &&\forall v,k
    %\label{LP:1comm} 
    %\\
    &C_v \ge C_u + \groupdelay k \cdot (x_{v,k} - z_{u,v,k} ) &&\forall u,v,k: u \prec v 
    \label{LP:delay} 
    \\
    &C_v \ge C_u + \sum_k x_{v,k} &&\forall u,v: u \prec v
    \label{LP:precedence} 
    \\
    &\alpha \groupdelay k \ge \sum_u z_{u,v,k} &&\forall v,k
    \label{LP:duplicates}
}{
    &\sum_{k} x_{v,k} = 1 &&\forall v
    \label{LP:execution}
    \\[.35em]
    &C_v \ge 0 && \forall v
    \label{LP:mincompletion} 
    \\[.35em]
    &x_{v,k} \ge z_{u,v,k} &&\forall u,v, k
    \label{LP:minexecution} 
    \\[.35em]
    &y_{u,k} \ge x_{u,k} &&\forall u,k
    \label{LP:place} 
    \\[.35em]
    &y_{u,k} \ge z_{u,v,k} &&\forall u,v,k
    \label{LP:dup-place} 
    \\[.35em]
    &z_{u,v,k} \ge 0 &&\forall u,v,k
    \label{LP:mindup} 
}

%\smallskip
\BfPara{Variables} 
$\Calpha$ represents the makespan of the schedule. For each job $v$, $C_v$ represents the earliest completion time of $v$. For each job $v$ and group $\group k$, $x_{v,k}$ indicates whether or not $v$ is first executed on a machine in group $\group k$. For each $\group k$ and pair of jobs $u,v$ such that $u \prec v$, $z_{u,v,k}$ indicates whether $v$ is first executed on a machine in group $\group k$ and the earliest execution of $u$ is less that $\groupdelay k$ time before the execution of $v$.  Intuitively, $z_{u,v,k}$ indicates whether there must be a copy of $u$ executed on the same machine that first executes $v$. For each job $v$ and group $\group k$, $y_{v,k}$ indicates whether $x_{v,k} = 1$ or $z_{u,v,k} = 1$ for some $u$; that is, whether or not some copy of $u$ must be placed on group $\group k$. Note that constraints~(\ref{LP:mincompletion} - \ref{LP:mindup}) guarantee that all variables are non-negative. 


\smallskip
\BfPara{Makespan (\ref{LP:load}, \junk{\ref{LP:1comm},} \ref{LP:makespan})}
Constraint~\ref{LP:load} states that the makespan is at least the load on any single group. 
%Constraint~\ref{LP:1comm} states that we require at least one round of communication to any machine that executes even a single job. This allows us to minimize the additive term in our asymptotic bound.
Constraint~\ref{LP:makespan} states that the makespan is at least the maximum completion time of any job.


\smallskip
\BfPara{Machine delays (\ref{LP:delay}, \ref{LP:duplicates})}
Constraint~\ref{LP:delay} states that the earliest completion time of $v$ must be at least $\groupdelay k$ after the earliest completion time of any predecessor $u$ if $v$ is first executed on a machine in group $\group k$ and no copy of $u$ is duplicated on the same machine as $v$.  Constraint~\ref{LP:duplicates} limits the amount of duplication that can be done to improve the completion time of any job: if $v$ first executes on a machine in group $\group k$ at time $t$, then the number of predacessors that may be executed in the $\groupdelay k$ steps preceding $t$ is at most $\groupdelay k$. 

The remaining constraints enforce standard scheduling conditions. Constraint~\ref{LP:precedence} states that the completion time of $v$ is at least the completion time of any of its predecessors, and constraint~\ref{LP:execution} ensures that every job is executed on some group.  Constraints~\ref{LP:execution}, \ref{LP:minexecution} guarantee that $z_{u,v,k} \le 1$ for all $u,v,k$. This is an important feature of the LP, since a large $z$-value could be used to disproportionately reduce the delay between two jobs in constraint~\ref{LP:delay}. 



\begin{lemma}{\textbf{(\LP 1 is a valid relaxation)}}
    The minimum of $\C 1$ is at most $\opt$.
\label{lem:LP_valid}
\end{lemma}
\begin{proof}
    Consider an arbitrary schedule $\sigma$. Let $\Csigma$ be the makespa of $\sigma$, i.e.\ $\Csigma = \max_{v,i,t}\{ t: (i,t) \in \sigma(v)\}$. %We assume the schedule is \textit{minimal} in the sense that a job is executed at most once on any machine and no job is executed on any machine after the result of that job is available to the machine. It is easy to see that if $\sigma$ is not minimal, there exists a minimal schedule $\sigma'$ such that $\makespan{\sigma'} \le \makespan{\sigma}$. We give a solution to the LP in which $D = \makespan{\sigma} + \delay{\sigma}$.
    
    \smallskip
    \BfPara{LP solution} Set $\Calpha = \Csigma$. For each job $v$, set $C_v$ to be the earliest completion time of $v$ in $\sigma$, i.e.\ $C_v = \min_{i,t}\{t : (i,t) \in \sigma(v)\}$. Set $x_{v,k} = 1$ if $\group k$ is the group that contains the machine on which $v$ first completes (choosing arbitrarily if there is more than one) and set $x_{v,k'} = 0$ otherwise. For $u,v,k$, set $z_{u,v,k} = 1$ if $u \prec v$, $x_{v,k} = 1$, and $C_v - C_u < \groupdelay k$ (0 otherwise). Set $y_{u,k} = \max\{x_{u,k}, \max_v \{ z_{u,v,k} \}\}$.
    
    \smallskip
    \BfPara{Feasibility} We now establish that the solution defined is feasible. Constraints (\ref{LP:makespan}, \ref{LP:mincompletion} - \ref{LP:mindup}) are easy to verify. We first establish constraint~\ref{LP:load}. Consider constraint~\ref{LP:load} for fixed group $\group k$. $\sum_v y_{v,k}$ is upper bound by the total load $L$ on $\group k$. The constraint follows from $\Calpha \ge \Csigma \ge L / |\group k|$.
    %For fixed $v,k$, constraint~\labelcref{LP:1comm} holds by assignment of $D$ and definition of $\delay{\sigma}$.
    
    Consider constraint~\ref{LP:delay} for fixed $u,v,k$ where $u \prec v$. Let $X = x_{v,k}$ and let $Z = z_{u,v,k}$. If $(X,Z) = (0,0), (0,1)$, or $(1,1)$ then the constraint follows from constraint~\ref{LP:precedence}. Suppose $(X,Z) = (1,0)$. By assignment of $z_{u,v,k}$ we can infer that $C_v - C_u \ge \groupdelay k$, which shows the constraint is satisfied.
    
    Consider constraint~\ref{LP:duplicates} for fixed $v,k$. If $x_{v,k} = 0$ then the result follows from the fact that $z_{u,v,k} = 0$ for all $u$. If $x_{v,k} =  1$ then at most $\groupdelay k$ predacessors of $v$ that can be scheduled in the $\groupdelay k$ time before $C_v$. So the constraint is satisfied.  
\end{proof}


\subsection{Deriving a rounded solution to the linear program}
\label{sec:round}

\begin{definition}
    $(C,x,y,z)$ is a \emph{rounded solution} to \LP a if all values of $x,y,z$ are either 0 or 1. 
\end{definition}

Let \LP 1 be defined over groups $\group 1, \group 2, \ldots, \group{K}$. Given a solution $(\hat C, \hat x, \hat y, \hat z)$ to \LP 1, we construct an integer solution $(C,x,y,z)$ to \LP{2K} as follows. For each $v,k$, set $x_{v,k} = 1$ if $k = \max_{k'}\{\hat x_{v,k'}\}$ (if there is more than one maximizing $k$, arbitrarily select one); set to 0 otherwise. Set $z_{u,v,k} = 1$ if $x_{v,k} = 1$ and $\hat z_{u,v,k} \ge 1/(2K)$; set to 0 otherwise. For all $u,k$, $y_{u,k} = \max\{ x_{u,k}, \max_v \{z_{u,v,k}\}\}$. Set $C_v = 2K \cdot \hat C_v$. Set $C_{2K} = 2K \cdot \hat C_1$. 

\begin{lemma}
    If $(\hat C, \hat x, \hat y, \hat z)$ is a valid solution to \LP 1, then  $(C,x,y,z)$ is a valid solution to \LP{2K}. 
\label{lem:LPK_solution}
\end{lemma}
\begin{proof}
    By constraint~\ref{LP:execution}, $\sum_{k} \hat x_{v,k}$ is at least 1, so $\max_{k} \{\hat x_{v,k}\}$ is at least $1/K$.  Therefore, $x_{v,k} \le K \hat{x}_{v,k}$ for all $v$ and $k$. Also, $z_{u,v,k} \le 2K \hat z_{u,v,k}$ for any $u,v,k$ by definition. By the setting of $C_v$ for all $v$, $y_{v,k}$ for all $v,k$, and $C_{2K}$, it follows that constraints~(\ref{LP:makespan}, \ref{LP:precedence}-\ref{LP:mindup}) of \LP{1} imply the respective constraints of \LP{2K}.
    We first establish constraint~\labelcref{LP:load}. For any fixed group $\group k$,
    \begin{align*}
        2K \hat{C}_1 \cdot |\group k| &\ge 2K \sum_v \hat y_{v,k} = 2K \sum_v \max\{ \hat x_{v,k}, \max_u \{ \hat z_{v,u,k}\} \}  &&\by{constraints~\ref{LP:load}, \ref{LP:mindup} of \LP 1} \\
        &\ge 2K \sum_v \frac{\hat x_{v,k} + \max_u \{ \hat z_{v,u,k} \}}{2} \\
        &\ge 2K \sum_v \frac{ x_{v,k} + \max_u \{ z_{v,u,k} \}}{2K} \ge \sum_v y_{v,k} &&\by{definition of $y_{v,k}$} 
    \end{align*}
    which entails constraint~\ref{LP:load} by $C_{2K} = 2K \hat C_1$.
   % Since $z_{u,v,k}$ is 1 only if $x_{v,k}$ is 1, constraint~(\ref{LP:minexecution}) of \LP{2K} holds.
    %By definition, $z_{u,v,k} \le 2K \hat{z}_{u,v,k}$, implying that constraints~(\ref{LP*:load}) and~(\ref{LP*:nonneg}) of \LP{2K} also hold.  
    It remains to establish constraint~\labelcref{LP:delay} for fixed $u,v,k$.  We consider two cases.  If $\hat{x}_{v,k} < 1/K$, then $x_{v,k} = 0$, so the constraint is trivially true in \LP{2K}.  Otherwise, $x_{v,k} - z_{u,v,k}$ equals $1 - z_{u,v,k}$, which is 1 only if $x_{v,k} - z_{u,v,k}$ is at least $1/(2K)$.  This establishes constraint~\labelcref{LP:delay} of \LP{2K} and completes the proof of the lemma.
\end{proof}

\begin{lemma}
    $C_{2K} \le 4  K \cdot \opt$.
\label{lem:LPK_makespan}
\end{lemma}
\begin{proof}
    Lemma~\ref{lem:group_rounding} shows that our grouping of machines does not increase the value of the LP by more than a factor of 2. Therefore, by Lemma~\ref{lem:LP_valid}, $C_{2K} = 2K \cdot \hat C_1 \le 4 K \cdot \opt$. 
\end{proof}




\subsection{Computing a schedule given an integer solution to the LP}
\label{sec:schedule}

Suppose we are given a partition of $M$ into $K$ groups such that group $\group k$ is composed of identical machines (i.e. for all $i,j \in \group k$, $\delay i = \delay j$). We are also given a valid integer solution $(C,x,y,z)$ to \LP a defined over $\group 1, \ldots, \group K$. In this section, we show that we can construct a schedule that achieves an approximation for machine delays in terms of $\alpha$ and $K$. The combinatorial subroutine that constructs the schedule is defined in Algorithm~\ref{alg:scheduler}.

We define the Uniform Delay Precedence-constrained Scheduling (\udps) problem to be identical to machine delays except that, for all $i,j$, $\delay i = \delay j$. In Appendix~\ref{sec:uniform}, we give an algorithm \udps-Solver for \udps.


\begin{algorithm}
\setstretch{1.25}
\KwInit{$\forall v, \ \sigma(v) \gets \varnothing;\ T \gets 0$}
\While{$T \le \Calpha$}{
    \ForAll{groups $\group k$}{
        \If{for some integer $d$, $T = d \groupdelay k$}{
            $V_{k,d} \gets \{v: x_{v,k} = 1$ and $T \le C_v < T+ \groupdelay k \} $\;
            $U_{k,d} \gets \{u : \exists v \in V_{k,d},\  u \prec v$ and $T \le C_u < T + \groupdelay k \}$\;
            $\sigma' \gets $ \udps-Solver on $(V_{k,d} \cup U_{k,d}, \group{k})$\;
            $\forall v,i,t,\ $ if $(i,t) \in \sigma'(v)$ then $\sigma(v) \gets \sigma'(v) + \max_{u,j,t'} \{t: (j,t') \in \sigma(u)\} +   \groupdelay k$ \label{line:append}\;
        }
    }
    $T \gets T + 1$\;
}
\caption{Machine Delay Scheduling with Duplication}
\label{alg:scheduler}
\end{algorithm}


We now describe Algorithm~\ref{alg:scheduler} informally. The subroutine takes as input the integer variable assignments $(C,x,y,z)$ and initializes an empty schedule $\sigma$ and global parameter $T$ to 0. For a fixed value of $T$, we check each group $\group k$ to see whether there is some integer $d$ such that $T = d \groupdelay k$. If so, we define $V_{k,d}$ to be the set of jobs $v$ such that $x_{v,k} = 1$ and $T \le C_v < T + \groupdelay k$. We define $U_{v,k}$ to be the set of jobs $u$ such that, for some job $v \in V_{k,d}$, we have $u \prec v$ and $T \le C_u \le t + \groupdelay k$. We then run \udps-Solver on jobs $V_{k,d} \cup U_{k,d}$ using machines in $\group k$ and append the resulting schedule to $\sigma$. Once all groups $\group k$ have been checked, we increment $T$ and repeat until all jobs are scheduled. The structure of the schedule produced by Algorithm~\ref{alg:scheduler} is depicted in Figure~\ref{fig:schedule_structure}.


The following lemma provides guarantees for \udps-Solver. The lemma is entailed by Lemma~\ref{lem:udps}, proved in Appendix~\ref{sec:uniform}.
\begin{lemma}
    Let $U$ be a set of jobs such that for any $v \in U$ the number of predecessors of $v$ in $U$ (i.e., $|\{ u \prec v\} \cap U|$) is at most $\alpha \groupdelay k$. Then given as input the set $U$ of jobs and the set $\group k$ of identical machines, \udps-Solver produces, in polynomial time, a valid schedule with makespan less than $3\log(\alpha \groupdelay k )\alpha \bar{\rho}_k + \frac{2 \cdot |U|}{|\group k|}$.
\label{lem:uniform}
\end{lemma}


\begin{lemma}
    Algorithm~\ref{alg:scheduler} outputs a valid schedule in polynomial time.
\end{lemma}
\begin{proof}
    It is easy to see that the algorithm runs in polynomial time, and Lemma~\ref{lem:uniform} entails that precedence constraints are obeyed on each machine. Consider a fixed $v,k,d$ such that $v \in V_{k,d}$. By line~\ref{line:append}, we insert a communication phase of length $\groupdelay k$ before appending any schedule on group $\group k$. So, by the time Algorithm~\ref{alg:scheduler} executes any job in $V_{k,d}$, every job $u$ such that $C_u < d \groupdelay k$ is available to every machine in group $\group k$. So the only predecessors of $v$ left to execute are those jobs in $U_{k,d}$. Therefore, all communication constraints are satisfied.
\end{proof}



\begin{lemma}
    If $(C,x,y,z)$ is a valid solution to \LP a and $\Calpha \le \beta \cdot \opt$, then Algorithm~\ref{alg:scheduler} outputs a schedule with makespan at most $7\alpha\beta K \cdot \log (\alpha n) \cdot (\opt + \delay{})$ for any schedule $\sigma$.
\label{lem:integer_approximation}
\end{lemma}
\begin{proof}
    Fix any schedule $\sigma$. Note that the schedule produced by the algorithm executes jobs on one group at a time. Since there are $K$ groups, we need only to show that the amount of time spent executing jobs on any group is at most $7\alpha \beta \log (\alpha n) \cdot (\opt + \delay{})$.
    
    \begin{claim}
    \label{clm:z}
    For any $u,k,d$, if $u$ is in  $U_{k,d}$, then for some $v$ in $V_{k,d}$ we have $z_{u,v,k} = 1$. 
    \end{claim}
    \begin{proof}
    Fix a job $u$.  If $u$ is in $U_{k,d}$, then by the definition of $U_{k,d}$, there exists a job $v$ in $V_{k,d}$ such that $u \prec v$ and $T \le C_u < T + \groupdelay k$, where $T = d \groupdelay k$.  By the definition of $V_{k,d}$, $x_{v,k}$ is 1 and $T \le C_v < T + \groupdelay k$. Therefore, $C_v - C_u < \groupdelay k$.  By constraint~\ref{LP:delay}, $C_v \ge C_u + \groupdelay k (1 - z_{u,v,k})$, implying that $z_{u,v,k}$ cannot equal 0.  Since $z_{u,v,k}$ is either 0 or 1, we have $z_{u,v,k} = 1$.
    \end{proof}
    
    \begin{claim}
    \label{clm:chain}
    For any $v,k,d$, if $v \in V_{k,d}$ then $|\{u \prec v: u \in V_{k,d} \cup U_{k,d}\}|$ is at most $\alpha \groupdelay k$.% and the longest chain in $U_{k,d}$ has length at most $\alpha \groupdelay k$.
    \end{claim}
    \begin{proof} 
    Fix $v$ and consider any $u$ in $V_{k,d} \cup  U_{k,d}$ such that $u \prec v$.  
    By Claim~\ref{clm:z}, $z_{u,v,k} = 1$.  Therefore, $|\{u \prec v: u \in V_{k,d} \cup U_{k,d}\}|$ equals the right-hand side of constraint~\ref{LP:duplicates}, and hence at most $\alpha \groupdelay k$. 
    \end{proof}
        
    \begin{claim}
    \label{clm:D}
    For any $k$, $|\bigcup_d V_{k,d} \cup U_{k,d}| \le 2\Calpha \cdot |\group k|$.
    \end{claim} 
    \begin{proof} 
    Fix a $k$.  For any $v$ in $V_{k,d}$ we have $x_{v,k}=1$ by the definition of $V_{k,d}$.  Consider any $u$ in $U_{k,d}$.  By Claim~\ref{clm:z}, there exists a $v$ in $V_{k,d}$ such that $z_{u,v,k}$ equals 1; fix such a $v$.  By constraint~\ref{LP:dup-place}, $y_{u,k}$ equals 1.  Thus, $|\bigcup_d V_{k,d} \cup U_{k,d}|$ is at most twice the right-hand side of constraint~\ref{LP:load}, which is at most  $2\Calpha \cdot |\group k|$.
    \end{proof}
    
    So, by Lemma~\ref{lem:uniform} and Claim~\ref{clm:chain}, the total time spent executing jobs on a single group is upper bounded by
    \begin{align*}
        \sum_d \Big( 3 \log(\alpha \groupdelay k)  \alpha \groupdelay k + \frac{2 \cdot |V_{k,d} \cup U_{k,d}|}{|\group k|} \Big) &= \ceil{\frac{D}{\groupdelay k}}  3\alpha \groupdelay k \log(\alpha \groupdelay k)  + \frac{2\sum_d |V_{k,d} \cup U_{k,d}|}{|\group k|}  \\
        &\le \left( \frac{D}{\groupdelay k} + 1 \right) 3\alpha \groupdelay k \log(\alpha \groupdelay k)  + \frac{4\Calpha \cdot  |\group k|}{|\group k|}   \\
        &\le 7\Calpha \alpha  \log(\alpha \groupdelay k) +  3\alpha \groupdelay k \log(\alpha \groupdelay k)  
    \end{align*}
    where the second line follows by Claim~\ref{clm:D}. Summing over all $k$, the total time in the schedule is at most $5KD\alpha \log(\alpha \rho m)$. The lemma follows from the fact that $\Calpha \le \beta \cdot (\makespan{\sigma} + \delay{\sigma})$ and $\groupdelay k \le n$.
\end{proof}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{Figures/schedule2.pdf}
    \caption{Structure of the schedule produced by Algorithm~\ref{alg:scheduler}. $\sigma_{k,d}$ denotes a schedule of $V_{k,d}$ on the machines in group $\group k$. The algorithm scans the $\text{LP}_{\alpha}$ solution by increasing time (left to right). At the start of each $V_{k,d}$, the algorithm constructs a schedule of the set and appends it to the existing schedule.}
    \label{fig:schedule_structure}
\end{figure}

\begin{theorem}
    There exists an algorithm to compute a schedule with makespan $O(K^3 \log n \cdot (\opt + \delay{}))$ in polynomial time.
\end{theorem}
\begin{proof}
    Lemma~\ref{lem:LPK_solution} entails that $(C,x,y,z)$ is a valid solution to \LP{2K}. Lemma~\ref{lem:LPK_makespan} entails that $\Calpha \le 4K \cdot \opt$. With $\alpha = 2K$ and $\beta = 4K$,  Lemma~\ref{lem:integer_approximation}  entails that the makespan of our schedule is at most
    \begin{align*}
        7K \cdot 2K \cdot 4K \cdot \log(2Kn) \cdot (\opt + \delay{}) &= 28K^3 \cdot (1 + \log K + \log n) \cdot (\opt + \delay{}) \\
        &\le 28K^3 \cdot (1 + \log\log n + \log n) \cdot (\opt + \delay{}) &&\by{def.\ of } K\\
        &\le 84K^3 \cdot \log n \cdot (\opt + \delay{}) 
    \end{align*}
    This proves the theorem.
\end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> STOC 23/model.tex <==
\section{Model and preliminaries}

\BfPara{Jobs and machines}
Let $V$ denote a set of $n$ unit-size jobs, partially-ordered according to $\prec$.  For any jobs $u$ and $v$ such that $u \prec v$, we refer to $u$ as a \emph{predecessor} of $v$.  Let $M$ denote a set of $m$ machines. We associate with each machine $i \in M$,  an integer \emph{size} $m_i \ge 1$ indicating the number of processors in $i$, an integer speed $s_i \ge 1$ for each processor of $i$, integer \emph{in-delay} of $\delayin {i}$, and integer \emph{out-delay} of $\delayout {i}$.  

\smallskip
\BfPara{Schedules}
A schedule $\sigma$ assigns a set of machine-time pairs to each job. If $(i,t) \in \sigma(v)$, this indicates that $v$ is executed on machine $i$ at time $t$. By default, this allows schedules to duplicate jobs; so, for a given job $v$, $\sigma(v)$ may contain multiple machine-time pairs for distinct machines $i$ and $j$.  In a \emph{no-duplication} schedule, $\sigma(v)$ contains exactly one machine-time pairs. Preemption is not allowed. For any job $v$ machine $i$ and time $t$, we say that $v$ is \textit{available} to $i$ at time $t$ if $v$ is executed on $i$ before time $t$ or on any machine $j$ before time $t - (\delayin i + \delayout j)$. If $v$ is scheduled at time $t$ on machine $i$, then all of its predecessors must be available to $i$ by time $t$. The number of jobs that can be executed on any $i$ at any time $t$ is at most $m_i$. The time to process a single job on any machine $i$ is $1/s_i$. 

Given a set of jobs and machines as above, we let \mdps\ denote the problem of determining a schedule that minimizes the \textit{makespan}, which is the maximum completion time of any job in the schedule. 

\smallskip
\BfPara{Reduction to in-delays}
We first show that \mdps\ reduces to the special case of \mdps\ with zero out-delays. 
This allows us to focus on \mdps\ with zero out-delays in the remainder of the paper.

\begin{lemma}
    For any $\alpha \ge 1$, a polynomial-time $\alpha$-approximation algorithm for \mdps\ (resp., \mdps\ without duplication) in which all out-delays are 0 implies a polynomial-time $\alpha$-approximation for \mdps\ (resp., \mdps\ without duplication).
    \label{lem:reduction}
\end{lemma}
\begin{proof}
    Let $\I$ be an instance of \mdps. We prove the lemma by showing the existence of polynomial-time computable functions $f$ and $f_{\I}$ with the following properties:
    \begin{enumerate*}[label={\bf\small(\alph*)}]
        \item $f(\I)$ is an instance of \mdps\ in which all out-delays are 0, \label{red:indelay}
        \item the optimal makespan of $\I$ is at least the optimal makespan of $f(\I)$, and \label{red:opt}
        \item if $\sigma$ is a schedule (resp., no-duplication schedule) of $f(\I)$ then $f_{\I}(\sigma)$ is a schedule of $\I$ (resp., no-duplication) with the same makespan. \label{red:inverse}
    \end{enumerate*}
    The existence of these functions is sufficient to prove the lemma. For a given schedule $\sigma$ and arbitrary job $v$ and machine $i$, we define $t^{\sigma}_{v,i}$ to be the execution time of $v$ on machine $i$ according to $\sigma$.  
    We first define the instance $f(\I)$ in which all out delays are 0. Since there are no out-delays, we use $\rho_i$ to denote the in-delay of an arbitrary machine $i$ in instance $f(\I)$; $\delayin i$ and $\delayout i$, respectively, denote the in- and out-delay of $i$ in $\I$. $f(\I)$ is identical to $\I$ except that, for each machine $i$, the out-delay of $i$ is 0 and the in-delay $\rho_i$ is equal to $\delayin i + \delayout i$. It is easy to see that $f$ is polynomial-time computable and has property \ref{red:indelay}. 
    
    We show that $f$ has property \ref{red:opt}. Consider a schedule $\sigma$ of $\I$. We construct a schedule $\sigma'$ of $f(\I)$ with the same makespan. For any job $v$ and machine $i$, if $v$ is executed on $i$ at time $t$ according to $\sigma$, then $v$ is executed on $i$ at time $t + \delayout i$ in $\sigma'$. It is easy to see that the makespan (the time at which the result of all jobs is available to the central machine) is the same for both $\sigma$ and $\sigma'$. It is also easy to see that the ordering of jobs on a single machine is maintained in $\sigma'$. So we must only show that the communication constraints are satisfied. Consider two jobs $u$ and $v$ such that $u \prec v$, $u$ is executed on $i$ and $v$ is executed on $j \ne i$, and $t^{\sigma}_{v,j} - t^{\sigma}_{u,i} \ge \delayout i + \delayin j$. Then $t^{\sigma'}_{v,j} - t^{\sigma'}_{u,i} = (t^{\sigma}_{v,j} + \delayout j) - (t^{\sigma}_{u,i} + \delayout i) \ge \delayout i + \delayin j + \delayout j - \delayout i = \delayin j + \delayout j = \rho_j$, implying that $\sigma'$ is a valid schedule of $f(\I)$.   Therefore, property \ref{red:opt} holds.   
    
    We now define $f_{\I}$, which uses similar reasoning as above. Consider a schedule $\sigma$ of $f(\I)$. We define $f_{\I}(\sigma)$ to be schedule $\sigma'$, constructed as follows. For any job $v$ and machine $i$, if $v$ is executed on $i$ at time $t$ according to $\sigma$, then $v$ is executed on $i$ at time $t - \delayout i$ according to $\sigma'$. Note that the definition ensures that if $\sigma$ is a no-duplication schedule, then so is $\sigma'$.  Again, it is easy to see that $f_{\I}$ is polynomial-time computable, that the makespan is the same for both schedules, and that precedence constraints are maintained on individual machines. So consider two jobs $u$ and $v$ such that $u \prec v$, $u$ is executed on $i$ and $v$ is executed on $j \ne i$, and $t^{\sigma}_{v,j} - t^{\sigma}_{u,i} \ge \rho_j = \delayin j + \delayout j$. Then $t^{\sigma'}_{v,j} - t^{\sigma'}_{u,i} = (t^{\sigma}_{v,j} - \delayout j) - (t^{\sigma}_{u,i} - \delayout i) \ge \delayin j + \delayout j - \delayout j + \delayout i = \delayin j + \delayout i$, implying that $\sigma'$ is a valid schedule of $\I$.   Therefore, property \ref{red:inverse} holds.  
\end{proof}

%Throughout the paper, when machines are divided into groups of identical machines, we use $\bar{\rho}_k$ and $\bar m_k$ to denote, respectively, the in-delay and size of all machines in the group with index $k$.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

